The Disk Wind in the Neutron Star Low-mass X-Ray Binary GX 13+1

We present the analysis of seven \emph{Chandra} High Energy Transmission Grating Spectrometer and six simultaneous \emph{RXTE} Proportional Counter Array observations of the persistent neutron star (NS) low-mass X-ray binary GX 13+1 on its normal and horizontal branches. Across nearly 10 years, GX 13+1 is consistently found to be accreting at $50-70$\% Eddington, and all observations exhibit multiple narrow, blueshifted absorption features, the signature of a disk wind, despite the association of normal and horizontal branches with jet activity. A single absorber with standard abundances cannot account for all seven major disk wind features, indicating that multiple absorption zones may be present. Two or three absorbers can produce all of the absorption features at their observed broadened widths and reveal that multiple kinematic components produce the accretion disk wind signature. Assuming the most ionized absorber reflects the physical conditions closest to the NS, we estimate a wind launching radius of $7\times10^{10}$ cm, for an electron density of $10^{12}$ cm$^{-3}$. This is consistent with the Compton radius and also with a thermally driven wind. Because of the source's high Eddington fraction, radiation pressure likely facilitates the wind launching.

==> references.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Jessamyn Allen at 2018-06-21 17:39:36 -0700 


%% Saved with string encoding Unicode (UTF-8) 



@article{ponti18,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.473.2304P},
	Archiveprefix = {arXiv},
	Author = {{Ponti}, G. and {Bianchi}, S. and {Mu{\~n}oz-Darias}, T. and {Mori}, K. and {De}, K. and {Rau}, A. and {De Marco}, B. and {Hailey}, C. and {Tomsick}, J. and {Madsen}, K.~K. and {Clavel}, M. and {Rahoui}, F. and {Lal}, D.~V. and {Roy}, S. and {Stern}, D.},
	Date-Added = {2018-04-28 03:39:43 +0000},
	Date-Modified = {2018-04-28 03:39:43 +0000},
	Doi = {10.1093/mnras/stx2425},
	Eprint = {1709.06571},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, methods: observational, techniques: spectroscopic, stars: neutron, absorption lines, X-rays: binaries},
	Month = jan,
	Pages = {2304-2323},
	Primaryclass = {astro-ph.HE},
	Title = {{NuSTAR + XMM-Newton monitoring of the neutron star transient AX J1745.6-2901}},
	Volume = 473,
	Year = 2018,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stx2425}}

@article{bianchi17,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.472.2454B},
	Archiveprefix = {arXiv},
	Author = {{Bianchi}, S. and {Ponti}, G. and {Mu{\~n}oz-Darias}, T. and {Petrucci}, P.-O.},
	Date-Added = {2018-04-28 03:28:48 +0000},
	Date-Modified = {2018-04-28 03:28:48 +0000},
	Doi = {10.1093/mnras/stx2173},
	Eprint = {1709.00860},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, black hole physics, stars: neutron, stars: winds, outflows, X-rays: binaries, X-rays: individual: AX J1745.6-2901},
	Month = dec,
	Pages = {2454-2461},
	Primaryclass = {astro-ph.HE},
	Title = {{Photoionization instability of the Fe K absorbing plasma in the neutron star transient AX J1745.6-2901}},
	Volume = 472,
	Year = 2017,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stx2173}}

@article{murphy,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...797...12M},
	Archiveprefix = {arXiv},
	Author = {{Murphy}, K.~D. and {Nowak}, M.~A.},
	Date-Added = {2018-03-16 00:41:28 +0000},
	Date-Modified = {2018-03-16 00:41:28 +0000},
	Doi = {10.1088/0004-637X/797/1/12},
	Eid = {12},
	Eprint = {1406.4497},
	Journal = {\apj},
	Keywords = {galaxies: active, galaxies: individual: MCG+8-11-11, galaxies: Seyfert, X-rays: galaxies},
	Month = dec,
	Pages = {12},
	Primaryclass = {astro-ph.HE},
	Title = {{A Chandra-HETG View of MCG +8-11-11}},
	Volume = 797,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/797/1/12}}

@article{foreman,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013PASP..125..306F},
	Archiveprefix = {arXiv},
	Author = {{Foreman-Mackey}, D. and {Hogg}, D.~W. and {Lang}, D. and {Goodman}, J.},
	Date-Added = {2018-03-16 00:40:12 +0000},
	Date-Modified = {2018-03-16 00:40:12 +0000},
	Doi = {10.1086/670067},
	Eprint = {1202.3665},
	Journal = {\pasp},
	Month = mar,
	Pages = {306},
	Primaryclass = {astro-ph.IM},
	Title = {{emcee: The MCMC Hammer}},
	Volume = 125,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/670067}}

@article{done16,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.473..838D},
	Author = {{Done}, C. and {Tomaru}, R. and {Takahashi}, T.},
	Date-Added = {2018-03-06 07:22:36 +0000},
	Date-Modified = {2018-03-06 07:22:36 +0000},
	Doi = {10.1093/mnras/stx2400},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, black hole physics, magnetic fields, X-rays: binaries},
	Month = jan,
	Pages = {838-848},
	Title = {{Thermal winds in stellar mass black hole and neutron star binary systems}},
	Volume = 473,
	Year = 2018,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stx2400}}

@article{ryota18,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.tmp..332T},
	Archiveprefix = {arXiv},
	Author = {{Tomaru}, R. and {Done}, C. and {Odaka}, H. and {Watanabe}, S. and {Takahashi}, T.},
	Date-Added = {2018-03-03 07:19:19 +0000},
	Date-Modified = {2018-03-03 07:19:19 +0000},
	Doi = {10.1093/mnras/sty336},
	Eprint = {1802.07019},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, black hole physics, X-rays: binaries, X-ray: individual: (GX 13+1)},
	Month = feb,
	Primaryclass = {astro-ph.HE},
	Title = {{Monte-Carlo simulations of the detailed iron absorption line profiles from thermal winds in X-ray binaries}},
	Year = 2018,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/sty336}}

@article{rxtepca,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJS..163..401J},
	Author = {{Jahoda}, K. and {Markwardt}, C.~B. and {Radeva}, Y. and {Rots}, A.~H. and {Stark}, M.~J. and {Swank}, J.~H. and {Strohmayer}, T.~E. and {Zhang}, W.},
	Date-Added = {2018-02-13 05:20:59 +0000},
	Date-Modified = {2018-02-13 05:20:59 +0000},
	Doi = {10.1086/500659},
	Eprint = {astro-ph/0511531},
	Journal = {\apjs},
	Keywords = {Instrumentation: Detectors, Space Vehicles: Instruments},
	Month = apr,
	Pages = {401-423},
	Title = {{Calibration of the Rossi X-Ray Timing Explorer Proportional Counter Array}},
	Volume = 163,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/500659}}

@article{brandt2000,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...544L.123B},
	Author = {{Brandt}, W.~N. and {Schulz}, N.~S.},
	Date-Added = {2017-05-26 06:27:04 +0000},
	Date-Modified = {2017-05-26 06:27:04 +0000},
	Doi = {10.1086/317313},
	Eprint = {astro-ph/0007406},
	Journal = {\apjl},
	Keywords = {Accretion, Accretion Disks, Stars: Binaries: Close, Stars: Individual: Constellation Name: Circinus X-1, Stars: Neutron, Techniques: Spectroscopic, X-Rays: Stars},
	Month = dec,
	Pages = {L123-L127},
	Title = {{The Discovery of Broad P Cygni X-Ray Lines from Circinus X-1 with the Chandra High-Energy Transmission Grating Spectrometer}},
	Volume = 544,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/317313}}

@article{schulz2002,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...572..971S},
	Author = {{Schulz}, N.~S. and {Brandt}, W.~N.},
	Date-Added = {2017-05-26 00:32:44 +0000},
	Date-Modified = {2017-05-26 00:32:44 +0000},
	Doi = {10.1086/340369},
	Eprint = {astro-ph/0112483},
	Journal = {\apj},
	Keywords = {Accretion, Accretion Disks, Stars: Binaries: Close, Stars: Individual: Constellation Name: Circinus X-1, Stars: Neutron, Techniques: Spectroscopic, X-Rays: Stars},
	Month = jun,
	Pages = {971-983},
	Title = {{Variability of the X-Ray P Cygni Line Profiles from Circinus X-1 near Zero Phase}},
	Volume = 572,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/340369}}

@article{white86,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1986MNRAS.218..129W},
	Author = {{White}, N.~E. and {Peacock}, A. and {Hasinger}, G. and {Mason}, K.~O. and {Manzo}, G. and {Taylor}, B.~G. and {Branduardi-Raymont}, G.},
	Date-Added = {2017-05-25 17:13:02 +0000},
	Date-Modified = {2017-05-25 17:13:09 +0000},
	Doi = {10.1093/mnras/218.1.129},
	Journal = {\mnras},
	Keywords = {Astronomical Spectroscopy, Emission Spectra, K Lines, Metallic Stars, X Ray Binaries, Continuous Spectra, Exosat Satellite, Line Spectra, Proportional Counters, Stellar Mass},
	Month = jan,
	Pages = {129-138},
	Title = {{A study of the continuum and iron K line emission from low-mass X-ray binaries}},
	Volume = 218,
	Year = 1986,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/218.1.129}}

@article{asai2000,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000ApJS..131..571A},
	Author = {{Asai}, K. and {Dotani}, T. and {Nagase}, F. and {Mitsuda}, K.},
	Date-Added = {2017-05-25 16:29:24 +0000},
	Date-Modified = {2017-05-25 16:29:24 +0000},
	Doi = {10.1086/317374},
	Journal = {\apjs},
	Keywords = {Stars: Binaries: Close, Stars: Neutron, X-Rays: Stars},
	Month = dec,
	Pages = {571-591},
	Title = {{Iron K Emission Lines in the Energy Spectra of Low-Mass X-Ray Binaries Observed with ASCA}},
	Volume = 131,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/317374}}

@article{shidatsu,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...823..159S},
	Archiveprefix = {arXiv},
	Author = {{Shidatsu}, M. and {Done}, C. and {Ueda}, Y.},
	Date-Added = {2017-05-19 01:01:24 +0000},
	Date-Modified = {2017-05-19 01:01:24 +0000},
	Doi = {10.3847/0004-637X/823/2/159},
	Eid = {159},
	Eprint = {1604.04346},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, black hole physics, X-rays: binaries, X-rays: individual: GRO J1655{\ndash}40},
	Month = jun,
	Pages = {159},
	Primaryclass = {astro-ph.HE},
	Title = {{An Optically Thick Disk Wind in GRO J1655-40?}},
	Volume = 823,
	Year = 2016,
	Bdsk-Url-1 = {http://dx.doi.org/10.3847/0004-637X/823/2/159}}

@article{neilsencomptonthick,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...822...20N},
	Archiveprefix = {arXiv},
	Author = {{Neilsen}, J. and {Rahoui}, F. and {Homan}, J. and {Buxton}, M.},
	Date-Added = {2017-05-19 00:59:40 +0000},
	Date-Modified = {2017-05-19 00:59:40 +0000},
	Doi = {10.3847/0004-637X/822/1/20},
	Eid = {20},
	Eprint = {1603.04070},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, black hole physics, infrared: stars, stars: black holes, stars: winds, outflows},
	Month = may,
	Pages = {20},
	Primaryclass = {astro-ph.HE},
	Title = {{A Super-Eddington, Compton-thick Wind in GRO J1655-40?}},
	Volume = 822,
	Year = 2016,
	Bdsk-Url-1 = {http://dx.doi.org/10.3847/0004-637X/822/1/20}}

@article{tarter,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1969ApJ...156..943T},
	Author = {{Tarter}, C.~B. and {Tucker}, W.~H. and {Salpeter}, E.~E.},
	Date-Added = {2017-05-19 00:51:46 +0000},
	Date-Modified = {2017-05-19 00:51:46 +0000},
	Doi = {10.1086/150026},
	Journal = {\apj},
	Month = jun,
	Pages = {943},
	Title = {{The Interaction of X-Ray Sources with Optically Thin Environments}},
	Volume = 156,
	Year = 1969,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/150026}}

@article{ponti16,
	Author = {Ponti, G. and Bianchi, S. and Mu{\~n}oz-Darias, T. and De, K. and Fender, R. and Merloni, A.},
	Date-Added = {2017-05-18 16:09:31 +0000},
	Date-Modified = {2017-05-18 16:09:31 +0000},
	Doi = {10.1002/asna.201612339},
	Issn = {1521-3994},
	Journal = {Astronomische Nachrichten},
	Keywords = {accretion, accretion disks, stars: winds, outflows, techniques: spectroscopic, X-rays: binaries, X-rays: individuals (AX J1745.6-2901, EXO0748-676)},
	Number = {4-5},
	Pages = {512--517},
	Publisher = {WILEY-VCH Verlag},
	Title = {High ionisation absorption in low mass X-ray binaries},
	Url = {http://dx.doi.org/10.1002/asna.201612339},
	Volume = {337},
	Year = {2016},
	Bdsk-Url-1 = {http://dx.doi.org/10.1002/asna.201612339}}

@article{neilsen11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737...69N},
	Archiveprefix = {arXiv},
	Author = {{Neilsen}, J. and {Remillard}, R.~A. and {Lee}, J.~C.},
	Date-Added = {2017-05-18 15:57:49 +0000},
	Date-Modified = {2017-05-18 15:57:49 +0000},
	Doi = {10.1088/0004-637X/737/2/69},
	Eid = {69},
	Eprint = {1106.0298},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, binaries: close, black hole physics, instabilities, stars: winds, outflows, X-rays: individual: GRS 1915+105},
	Month = aug,
	Pages = {69},
	Primaryclass = {astro-ph.HE},
	Title = {{The Physics of the ``Heartbeat'' State of GRS 1915+105}},
	Volume = 737,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/737/2/69}}

@article{kotani2000,
	Abstract = {We have carried out a precise energy spectral analysis of the superluminal jet source GRS 1915+105 observed with ASCA six times from 1994 to 1999. The source was so bright that most SIS data suffered from event pileup. We have developed a new technique to circumvent the pileup effect, which enabled us to study the spectrum in detail and at high resolution (Δ E / E ≈ 2%). In the energy spectra of 1994 and 1995, resonant absorption lines of Ca XX Kα, Fe XXV Kα, Fe XXVI Kα, as well as blends of the absorption lines of Ni XXVII Kα + Fe XXV Kβ and Ni XXVIII Kα + Fe XXVI Kβ, were observed. Such absorption lines have not been found in other objects, except for iron absorption lines from GRO J1655-40, another superluminal jet source. We carried out a "curve of growth" analysis for the absorption lines and estimated column densities of the absorbing ions. We found that a plasma of moderate temperature (0.1-10 keV) and cosmic abundance cannot account for the observed large equivalent widths. The hydrogen column density of such plasma would be so high that the optical depth of Thomson scattering would be too thick ( N H ##IMG## [http://ej.iop.org/icons/Entities/gtrsim.gif] {gtrsim} 10 24 cm -2 ). We require either a very high kinetic temperature of the ions ( ##IMG## [http://ej.iop.org/icons/Entities/gtrsim.gif] {gtrsim} 100 keV) or extreme overabundances ( ##IMG## [http://ej.iop.org/icons/Entities/gtrsim.gif] {gtrsim} 100 Z ☉ ). In the former case, the ion column densities have reasonable values of 10 17 -10 18 cm -2 . We modeled the absorber as a photoionized disk which envelops the central X-ray source. Using a photoionization calculation code, we constrain physical parameters of the plasma disk, such as the ionization parameter, radius, and density. Estimated parameters were found to be consistent with those of a radiation-driven disk wind. These absorption line features may be peculiar to superluminal jet sources and related to the jet formation mechanism. Alternatively, they may be common characteristics of supercritical edge-on systems.},
	Author = {Taro Kotani and Ken Ebisawa and Tadayasu Dotani and Hajime Inoue and Fumiaki Nagase and Yasuo Tanaka and Yoshihiro Ueda},
	Date-Added = {2017-05-18 15:51:30 +0000},
	Date-Modified = {2017-05-18 15:51:30 +0000},
	Journal = {The Astrophysical Journal},
	Number = {1},
	Pages = {413},
	Title = {ASCA Observations of the Absorption Line Features from the Superluminal Jet Source GRS 1915+105},
	Url = {http://stacks.iop.org/0004-637X/539/i=1/a=413},
	Volume = {539},
	Year = {2000},
	Bdsk-Url-1 = {http://stacks.iop.org/0004-637X/539/i=1/a=413}}

@article{ueda98,
	Abstract = {We report the detection of iron K-absorption lines in the energy spectra of the superluminal jet source GRO J1655-40. We observed the source with ASCA on four occasions from 1994 through 1996. Significant absorption-line features were found at 6.63 $\pm$ 0.07 keV when the X-ray intensity was low (0.27-0.57 crab) and at 6.95 $\pm$ 0.10 keV when the intensity was high (2.2 crab). The former are interpreted as resonance absorption lines from helium-like iron and the latter are those from hydrogen-like iron, respectively. This gives direct evidence for the presence of highly ionized plasma in a nonspherical configuration in the vicinity of the black hole. The change of the ionization state of iron suggests that the plasma is photoionized by X-ray irradiation. The observed equivalent width (about 60 eV for the helium-like Kα line) and the ionization parameter ξ (~10 3 ) constrain the size of the plasma to ~10 10 cm. The similarity of these properties to those of the other superluminal source GRS 1915+105 may imply some connection between the presence of such highly ionized plasma and the formation of relativistic jets.},
	Author = {Y. Ueda and H. Inoue and Y. Tanaka and K. Ebisawa and F. Nagase and T. Kotani and N. Gehrels},
	Date-Added = {2017-05-18 15:49:36 +0000},
	Date-Modified = {2017-05-18 15:49:48 +0000},
	Journal = {The Astrophysical Journal},
	Number = {2},
	Pages = {782},
	Title = {Detection of Absorption-Line Features in the X-Ray Spectra of the Galactic Superluminal Source GRO J1655--40},
	Url = {http://stacks.iop.org/0004-637X/492/i=2/a=782},
	Volume = {492},
	Year = {1998},
	Bdsk-Url-1 = {http://stacks.iop.org/0004-637X/492/i=2/a=782}}

@article{millerigrj17480,
	Abstract = {Accretion disk winds are revealed in Chandra gratings spectra of black holes. The winds are hot and highly ionized (typically composed of He-like and H-like charge states) and show modest blueshifts. Similar line spectra are sometimes seen in "dipping" low-mass X-ray binaries (LMXBs), which are likely viewed edge-on; however, that absorption is tied to structures in the outer disk, and blueshifts are not typically observed. Here, we report the detection of blueshifted He-likeFe XXV (3100 $\pm$ 400 km s --1 ) and H-likeFe XXVI (1000 $\pm$ 200 km s --1 ) absorption lines in a Chandra /HETG spectrum of the transient pulsar and LMXB IGR J17480--2446 in Terzan 5. These features indicate a disk wind with at least superficial similarities to those observed in stellar-mass black holes. The wind does not vary strongly with numerous weak X-ray bursts or flares. A broad Fe K emission line is detected in the spectrum, and fits with different line models suggest that the inner accretion disk in this system may be truncated. If the stellar magnetic field truncates the disk, a field strength of B = (0.7-4.0)×10 9 G is implied, which is in line with estimates based on X-ray timing techniques. We discuss our findings in the context of accretion flows onto neutron stars and stellar-mass black holes.},
	Author = {Jon M. Miller and Dipankar Maitra and Edward M. Cackett and Sudip Bhattacharyya and Tod E. Strohmayer},
	Date-Added = {2017-05-10 01:15:09 +0000},
	Date-Modified = {2017-05-10 01:15:09 +0000},
	Journal = {The Astrophysical Journal Letters},
	Number = {1},
	Pages = {L7},
	Title = {A Fast X-ray Disk Wind in the Transient Pulsar IGR J17480--2446 in Terzan 5},
	Url = {http://stacks.iop.org/2041-8205/731/i=1/a=L7},
	Volume = {731},
	Year = {2011},
	Bdsk-Url-1 = {http://stacks.iop.org/2041-8205/731/i=1/a=L7}}

@article{miller12H1743,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...759L...6M},
	Archiveprefix = {arXiv},
	Author = {{Miller}, J.~M. and {Raymond}, J. and {Fabian}, A.~C. and {Reynolds}, C.~S. and {King}, A.~L. and {Kallman}, T.~R. and {Cackett}, E.~M. and {van der Klis}, M. and {Steeghs}, D.~T.~H.},
	Date-Added = {2017-05-10 00:29:32 +0000},
	Date-Modified = {2017-05-10 00:29:32 +0000},
	Doi = {10.1088/2041-8205/759/1/L6},
	Eid = {L6},
	Eprint = {1208.4514},
	Journal = {\apjl},
	Keywords = {accretion, accretion disks, black hole physics, X-rays: binaries},
	Month = nov,
	Pages = {L6},
	Primaryclass = {astro-ph.HE},
	Title = {{The Disk-wind-Jet Connection in the Black Hole H 1743-322}},
	Volume = 759,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/759/1/L6}}

@article{rochelobe,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...268..368E},
	Author = {{Eggleton}, P.~P.},
	Date-Added = {2017-05-05 00:57:40 +0000},
	Date-Modified = {2017-05-05 00:57:40 +0000},
	Doi = {10.1086/160960},
	Journal = {\apj},
	Keywords = {Binary Stars, Celestial Mechanics, Orbital Elements, Roche Limit, Mass Ratios, Radii},
	Month = may,
	Pages = {368},
	Title = {{Approximations to the radii of Roche lobes}},
	Volume = 268,
	Year = 1983,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/160960}}

@article{nsstates,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.443.3270M},
	Archiveprefix = {arXiv},
	Author = {{Mu{\~n}oz-Darias}, T. and {Fender}, R.~P. and {Motta}, S.~E. and {Belloni}, T.~M.},
	Date-Added = {2017-05-04 22:17:28 +0000},
	Date-Modified = {2017-05-04 22:17:28 +0000},
	Doi = {10.1093/mnras/stu1334},
	Eprint = {1407.1318},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, black hole physics, stars: black holes, stars: neutron, X-rays: binaries},
	Month = oct,
	Pages = {3270-3283},
	Primaryclass = {astro-ph.HE},
	Title = {{Black hole-like hysteresis and accretion states in neutron star low-mass X-ray binaries}},
	Volume = 443,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stu1334}}

@article{trigoboirin12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013AcPol..53..659D},
	Archiveprefix = {arXiv},
	Author = {{D{\'{\i}}az Trigo}, M. and {Boirin}, L.},
	Date-Added = {2017-05-04 16:47:43 +0000},
	Date-Modified = {2017-05-04 16:47:43 +0000},
	Eprint = {1210.0318},
	Journal = {Acta Polytechnica},
	Pages = {659},
	Primaryclass = {astro-ph.HE},
	Title = {{Disc Atmospheres and Winds in X-ray Binaries}},
	Volume = 53,
	Year = 2013}

@article{mhdwindmodel,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2017NatAs...1E..62F},
	Archiveprefix = {arXiv},
	Author = {{Fukumura}, K. and {Kazanas}, D. and {Shrader}, C. and {Behar}, E. and {Tombesi}, F. and {Contopoulos}, I.},
	Date-Added = {2017-05-04 00:49:54 +0000},
	Date-Modified = {2017-05-04 00:49:54 +0000},
	Doi = {10.1038/s41550-017-0062},
	Eid = {0062},
	Eprint = {1702.02197},
	Journal = {Nature Astronomy},
	Month = mar,
	Pages = {0062},
	Primaryclass = {astro-ph.HE},
	Title = {{Magnetic origin of black hole winds across the mass scale}},
	Volume = 1,
	Year = 2017,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/s41550-017-0062}}

@article{higproga17,
	Abstract = {A number of X-ray binaries exhibit clear evidence for the presence of disk winds in the high/soft state. A promising driving mechanism for these outflows is mass loss driven by the thermal expansion of X-ray heated material in the outer disk atmosphere. Higginbottom & Proga recently demonstrated that the properties of thermally driven winds depend critically on the shape of the thermal equilibrium curve, since this determines the thermal stability of the irradiated material. For a given spectral energy distribution, the thermal equilibrium curve depends on an exact balance between the various heating and cooling mechanisms at work. Most previous work on thermally driven disk winds relied on an analytical approximation to these rates. Here, we use the photoionization code cloudy to generate realistic heating and cooling rates which we then use in a 2.5D hydrodynamic model computed in ZEUS to simulate thermal winds in a typical black hole X-ray binary. We find that these heating and cooling rates produce a significantly more complex thermal equilibrium curve, with dramatically different stability properties. The resulting flow, calculated in the optically thin limit, is qualitatively different from flows calculated using approximate analytical rates. Specifically, our thermal disk wind is much denser and slower, with a mass-loss rate that is a factor of two higher and characteristic velocities that are a factor of three lower. The low velocity of the flow--- ##IMG## [http://ej.iop.org/images/0004-637X/836/1/42/apjaa55fdieqn1.gif] {${v}_{\max }\simeq 200$} km s −1 ---may be difficult to reconcile with observations. However, the high mass-loss rate---15 × the accretion rate---is promising, since it has the potential to destabilize the disk. Thermally driven disk winds may therefore provide a mechanism for state changes.},
	Author = {N. Higginbottom and D. Proga and C. Knigge and K. S. Long},
	Date-Added = {2017-05-03 19:05:00 +0000},
	Date-Modified = {2017-05-03 19:05:09 +0000},
	Journal = {The Astrophysical Journal},
	Number = {1},
	Pages = {42},
	Title = {Thermal Disk Winds in X-Ray Binaries: Realistic Heating and Cooling Rates Give Rise to Slow, but Massive, Outflows},
	Url = {http://stacks.iop.org/0004-637X/836/i=1/a=42},
	Volume = {836},
	Year = {2017},
	Bdsk-Url-1 = {http://stacks.iop.org/0004-637X/836/i=1/a=42}}

@article{xiang09,
	Abstract = {We present a detailed spectral study (photoionization modeling and variability) of the "Big Dipper"4U 1624--490 based on a Chandra -High Energy Transmission Grating Spectrometer (HETGS) observation over the ~76 ks binary orbit of 4U 1624--490 . While the continuum spectrum can be modeled using a blackbody plus power law, a slightly better fit is obtained using a single Γ = 2.25 power-law partially (71%) covered by a local absorber of column density ##IMG## [http://ej.iop.org/images/0004-637X/701/2/984/apj302903ieqn1.gif] {$N_{\rm H,\ Local}=8.1_{-0.6}^{+0.7}\times 10^{22}\, \rm cm^{-2}$} . The data show a possible quasi-sinusoidal modulation with period 43 +13 --9 ks that might be due to changes in local obscuration. Photoionization modeling with the XSTAR code and variability studies of the observed strong Fe XXV and Fe XXVI absorption lines point to a two-temperature plasma for their origin: a highly ionized component of ionization parameter ξ hot ##IMG## [http://ej.iop.org/icons/Entities/ap.gif] {≈} 10 4.3 erg cm s -1 ( T ~ 3.0 × 10 6 K) associated with an extended accretion disk corona of radius R ~ 3 × 10 10 cm, and a less-ionized more variable component of ξ ##IMG## [http://ej.iop.org/icons/Entities/ap.gif] {≈} 10 3.4 erg cm s -1 ( T ~ 1.0 × 10 6 K) and ##IMG## [http://ej.iop.org/images/0004-637X/701/2/984/apj302903ieqn2.gif] {$\rm \xi \approx 10^{3.1}\;erg\;cm\;s^{-1}$} ( T ~ 0.9 × 10 6 K) coincident with the accretion disk rim. We use this, with the observed Fe XXV and Fe XXVI absorption line variations (in wavelength, strength, and width) to construct a viewing geometry that is mapped to changes in plasma conditions over the4U 1624--490 orbital period.},
	Author = {Jingen Xiang and Julia C. Lee and Michael A. Nowak and J{\"o}rn Wilms and Norbert S. Schulz},
	Date-Added = {2017-05-03 15:58:41 +0000},
	Date-Modified = {2017-05-03 15:58:41 +0000},
	Journal = {The Astrophysical Journal},
	Number = {2},
	Pages = {984},
	Title = {The Accretion Disk Corona and Disk Atmosphere of 4U1624--490 as Viewed by the Chandra-High Energy Transmission Grating Spectrometer},
	Url = {http://stacks.iop.org/0004-637X/701/i=2/a=984},
	Volume = {701},
	Year = {2009},
	Bdsk-Url-1 = {http://stacks.iop.org/0004-637X/701/i=2/a=984}}

@article{homan16,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...830L...5H},
	Archiveprefix = {arXiv},
	Author = {{Homan}, J. and {Neilsen}, J. and {Allen}, J.~L. and {Chakrabarty}, D. and {Fender}, R. and {Fridriksson}, J.~K. and {Remillard}, R.~A. and {Schulz}, N.},
	Date-Added = {2017-05-02 19:45:38 +0000},
	Date-Modified = {2017-05-02 19:45:38 +0000},
	Doi = {10.3847/2041-8205/830/1/L5},
	Eid = {L5},
	Eprint = {1606.07954},
	Journal = {\apjl},
	Keywords = {accretion, accretion disks, stars: jets, stars: winds, outflows, X-rays: individual: GX 13+1},
	Month = oct,
	Pages = {L5},
	Primaryclass = {astro-ph.HE},
	Title = {{Evidence for Simultaneous Jets and Disk Winds in Luminous Low-mass X-Ray Binaries}},
	Volume = 830,
	Year = 2016,
	Bdsk-Url-1 = {http://dx.doi.org/10.3847/2041-8205/830/1/L5}}

@inproceedings{ciao,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006SPIE.6270E..1VF},
	Author = {{Fruscione}, A. and {McDowell}, J.~C. and {Allen}, G.~E. and {Brickhouse}, N.~S. and {Burke}, D.~J. and {Davis}, J.~E. and {Durham}, N. and {Elvis}, M. and {Galle}, E.~C. and {Harris}, D.~E. and {Huenemoerder}, D.~P. and {Houck}, J.~C. and {Ishibashi}, B. and {Karovska}, M. and {Nicastro}, F. and {Noble}, M.~S. and {Nowak}, M.~A. and {Primini}, F.~A. and {Siemiginowska}, A. and {Smith}, R.~K. and {Wise}, M.},
	Booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
	Date-Added = {2017-03-24 20:36:28 +0000},
	Date-Modified = {2017-03-24 20:36:28 +0000},
	Doi = {10.1117/12.671760},
	Eid = {62701V},
	Month = jun,
	Pages = {62701V},
	Series = {\procspie},
	Title = {{CIAO: Chandra's data analysis system}},
	Volume = 6270,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.671760}}

@article{miller08,
	Abstract = {We report on simultaneous Chandra HETGS and RXTE observations of the transient stellar-mass black hole GRO J1655--40, made during its 2005 outburst. Chandra reveals a line-rich X-ray absorption spectrum consistent with a disk wind. Prior modeling of the spectrum suggested that the wind may be magnetically driven, potentially providing insights into the nature of disk accretion onto black holes. In this paper, we present results obtained with new models for this spectrum, generated using three independent photoionization codes: XSTAR, Cloudy, and our own code. Fits to the spectrum in particular narrow wavelength ranges, in evenly spaced wavelength slices, and across a broad wavelength band all strongly prefer a combination of high density, high ionization, and small inner radius. Indeed, the results obtained from all three codes require a wind that originates more than 10 times closer to the black hole and carrying a mass flux that is on the order of 1000 times higher than predicted by thermal driving models. If seminal work on thermally driven disk winds is robust, magnetic forces may play a role in driving the disk wind in GRO J1655--40. However, even these modeling efforts must be regarded as crude given the complexity of the spectra. We discuss these results in the context of accretion flows in black holes and other compact objects.},
	Author = {J. M. Miller and J. Raymond and C. S. Reynolds and A. C. Fabian and T. R. Kallman and J. Homan},
	Date-Added = {2017-01-25 16:12:06 +0000},
	Date-Modified = {2017-01-25 16:12:06 +0000},
	Journal = {The Astrophysical Journal},
	Number = {2},
	Pages = {1359},
	Title = {The Accretion Disk Wind in the Black Hole GRO J1655--40},
	Url = {http://stacks.iop.org/0004-637X/680/i=2/a=1359},
	Volume = {680},
	Year = {2008},
	Bdsk-Url-1 = {http://stacks.iop.org/0004-637X/680/i=2/a=1359}}

@article{tgcat,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011AJ....141..129H},
	Author = {{Huenemoerder}, D.~P. and {Mitschang}, A. and {Dewey}, D. and {Nowak}, M.~A. and {Schulz}, N.~S. and {Nichols}, J.~S. and {Davis}, J.~E. and {Houck}, J.~C. and {Marshall}, H.~L. and {Noble}, M.~S. and {Morgan}, D. and {Canizares}, C.~R.},
	Date-Added = {2017-01-25 00:43:25 +0000},
	Date-Modified = {2017-01-25 00:43:25 +0000},
	Doi = {10.1088/0004-6256/141/4/129},
	Eid = {129},
	Journal = {\aj},
	Keywords = {catalogs, techniques: spectroscopic, X-rays: general},
	Month = apr,
	Pages = {129},
	Title = {{TGCat: The Chandra Transmission Grating Data Catalog and Archive}},
	Volume = 141,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/141/4/129}}

@article{isis,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000ASPC..216..591H},
	Author = {{Houck}, J.~C. and {Denicola}, L.~A.},
	Booktitle = {Astronomical Data Analysis Software and Systems IX},
	Date-Added = {2017-01-25 00:43:20 +0000},
	Date-Modified = {2017-01-25 00:43:20 +0000},
	Editor = {{Manset}, N. and {Veillet}, C. and {Crabtree}, D.},
	Pages = {591},
	Series = {Astronomical Society of the Pacific Conference Series},
	Title = {{ISIS: An Interactive Spectral Interpretation System for High Resolution X-Ray Spectroscopy}},
	Volume = 216,
	Year = 2000}

@article{homan04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...418..255H},
	Author = {{Homan}, J. and {Wijnands}, R. and {Rupen}, M.~P. and {Fender}, R. and {Hjellming}, R.~M. and {di Salvo}, T. and {van der Klis}, M.},
	Date-Added = {2016-10-14 16:39:57 +0000},
	Date-Modified = {2016-10-14 16:39:57 +0000},
	Doi = {10.1051/0004-6361:20034258},
	Eprint = {astro-ph/0309042},
	Journal = {\aap},
	Keywords = {accretion, accretion disks, stars: individual: GX 13+1, stars: neutron, ISM: jets and outflows, X-rays: binaries, radio continuum: stars},
	Month = apr,
	Pages = {255-263},
	Title = {{Simultaneous radio and X-ray observations of the low-mass X-ray binary GX 13+1}},
	Volume = 418,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20034258}}

@article{baukall01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJS..134..139B},
	Author = {{Bautista}, M.~A. and {Kallman}, T.~R.},
	Date-Added = {2016-10-14 00:11:48 +0000},
	Date-Modified = {2016-10-14 00:11:54 +0000},
	Doi = {10.1086/320363},
	Journal = {\apjs},
	Keywords = {Astronomical Data Bases: Miscellaneous, Atomic Data, Atomic Processes, Line: Formation, Ultraviolet: General, X-Rays: General},
	Month = may,
	Pages = {139-149},
	Title = {{The XSTAR Atomic Database}},
	Volume = 134,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/320363}}

@article{kallbau01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJS..133..221K},
	Author = {{Kallman}, T. and {Bautista}, M.},
	Date-Added = {2016-10-14 00:11:43 +0000},
	Date-Modified = {2016-10-14 00:12:04 +0000},
	Doi = {10.1086/319184},
	Journal = {\apjs},
	Keywords = {Atomic Processes, Radiation Mechanisms: Thermal, Radiative Transfer, Ultraviolet: General, X-Rays: General},
	Month = mar,
	Pages = {221-253},
	Title = {{Photoionization and High-Density Gas}},
	Volume = 133,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/319184}}

@article{canizares,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005PASP..117.1144C},
	Author = {{Canizares}, C.~R. and {Davis}, J.~E. and {Dewey}, D. and {Flanagan}, K.~A. and {Galton}, E.~B. and {Huenemoerder}, D.~P. and {Ishibashi}, K. and {Markert}, T.~H. and {Marshall}, H.~L. and {McGuirk}, M. and {Schattenburg}, M.~L. and {Schulz}, N.~S. and {Smith}, H.~I. and {Wise}, M.},
	Date-Added = {2016-10-13 23:45:44 +0000},
	Date-Modified = {2016-10-13 23:45:49 +0000},
	Doi = {10.1086/432898},
	Eprint = {astro-ph/0507035},
	Journal = {\pasp},
	Keywords = {space vehicles: instruments, Instrumentation: Spectrographs, X-Rays: General, methods: laboratory, Techniques: Spectroscopic},
	Month = oct,
	Pages = {1144-1171},
	Title = {{The Chandra High-Energy Transmission Grating: Design, Fabrication, Ground Calibration, and 5 Years in Flight}},
	Volume = 117,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/432898}}

@article{frank87,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1987A%26A...178..137F},
	Author = {{Frank}, J. and {King}, A.~R. and {Lasota}, J.-P.},
	Date-Added = {2016-10-13 22:44:15 +0000},
	Date-Modified = {2018-06-22 00:36:36 +0000},
	Journal = {\aap},
	Keywords = {Light Curve, Stellar Coronas, Stellar Mass Accretion, X Ray Binaries, Dipping, Eclipses, Ionization, Stellar Models},
	Month = may,
	Pages = {137-142},
	Title = {{The light curves of low-mass X-ray binaries}},
	Volume = 178,
	Year = 1987}

@article{giustini12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...758...70G},
	Archiveprefix = {arXiv},
	Author = {{Giustini}, M. and {Proga}, D.},
	Date-Added = {2016-10-12 16:58:58 +0000},
	Date-Modified = {2016-10-12 16:59:07 +0000},
	Doi = {10.1088/0004-637X/758/1/70},
	Eid = {70},
	Eprint = {1208.6044},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, black hole physics, line: formation, line: profiles},
	Month = oct,
	Pages = {70},
	Title = {{On the Diversity and Complexity of Absorption Line Profiles Produced by Outflows in Active Galactic Nuclei}},
	Volume = 758,
	Year = 2012,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUGJCVYJHZlcnNpb25YJG9iamVjdHNZJGFyY2hpdmVyVCR0b3ASAAGGoKgHCBMUFRYaIVUkbnVsbNMJCgsMDxJXTlMua2V5c1pOUy5vYmplY3RzViRjbGFzc6INDoACgAOiEBGABIAFgAdccmVsYXRpdmVQYXRoWWFsaWFzRGF0YV8QGC4uLy4uLy4uLy5UcmFzaC9pc2lzLmJpYtIXCxgZV05TLmRhdGFPEQFoAAAAAAFoAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAAAADKuP8USCsAADsdZbUIaXNpcy5iaWIAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAOwOl7dSs9SwAAAAAAAAAAAADAAIAAAkgAAAAAAAAAAAAAAAAAAAABi5UcmFzaAAQAAgAAMq5N1QAAAARAAgAANStO3wAAAABAAw7HWW1AAUe6gAAwCMAAgAyTWFjaW50b3NoIEhEOlVzZXJzOgBlbGVuYXRoZWRoZWw6AC5UcmFzaDoAaXNpcy5iaWIADgASAAgAaQBzAGkAcwAuAGIAaQBiAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIAIlVzZXJzL2VsZW5hdGhlZGhlbC8uVHJhc2gvaXNpcy5iaWIAEwABLwAAFQACABP//wAAgAbSGxwdHlokY2xhc3NuYW1lWCRjbGFzc2VzXU5TTXV0YWJsZURhdGGjHR8gVk5TRGF0YVhOU09iamVjdNIbHCIjXE5TRGljdGlvbmFyeaIiIF8QD05TS2V5ZWRBcmNoaXZlctEmJ1Ryb290gAEACAARABoAIwAtADIANwBAAEYATQBVAGAAZwBqAGwAbgBxAHMAdQB3AIQAjgCpAK4AtgIiAiQCKQI0Aj0CSwJPAlYCXwJkAnECdAKGAokCjgAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKQ},
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/758/1/70}}

@article{iaria06xb1916,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...647.1341I},
	Author = {{Iaria}, R. and {Di Salvo}, T. and {Lavagetto}, G. and {Robba}, N.~R. and {Burderi}, L.},
	Date-Added = {2016-10-12 15:28:57 +0000},
	Date-Modified = {2016-10-12 15:29:12 +0000},
	Doi = {10.1086/505616},
	Eprint = {astro-ph/0605055},
	Journal = {\apj},
	Keywords = {Line: Formation, Line: Identification, Stars: Individual: Alphanumeric: XB 1916-053, Stars: Neutron, X-Rays: Binaries, X-Rays: General},
	Month = aug,
	Pages = {1341-1348},
	Title = {{Chandra Observation of the Persistent Emission from the Dipping Source XB 1916-053}},
	Volume = 647,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/505616}}

@article{krolik81,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1981ApJ...249..422K},
	Author = {{Krolik}, J.~H. and {McKee}, C.~F. and {Tarter}, C.~B.},
	Date-Added = {2016-10-07 18:31:06 +0000},
	Date-Modified = {2016-10-07 18:31:11 +0000},
	Doi = {10.1086/159303},
	Journal = {\apj},
	Keywords = {Astronomical Models, Emission Spectra, Hydrogen Clouds, Quasars, Two Phase Flow, X Ray Sources, Compton Effect, Gas Temperature, Line Spectra, Phase Diagrams, Photoionization, Spectrum Analysis},
	Month = oct,
	Pages = {422-442},
	Title = {{Two-phase models of quasar emission line regions}},
	Volume = 249,
	Year = 1981,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUGJCVYJHZlcnNpb25YJG9iamVjdHNZJGFyY2hpdmVyVCR0b3ASAAGGoKgHCBMUFRYaIVUkbnVsbNMJCgsMDxJXTlMua2V5c1pOUy5vYmplY3RzViRjbGFzc6INDoACgAOiEBGABIAFgAdccmVsYXRpdmVQYXRoWWFsaWFzRGF0YV8QGC4uLy4uLy4uLy5UcmFzaC9pc2lzLmJpYtIXCxgZV05TLmRhdGFPEQFoAAAAAAFoAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAAAADKuP8USCsAADsdZbUIaXNpcy5iaWIAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAOwOl7dSs9SwAAAAAAAAAAAADAAIAAAkgAAAAAAAAAAAAAAAAAAAABi5UcmFzaAAQAAgAAMq5N1QAAAARAAgAANStO3wAAAABAAw7HWW1AAUe6gAAwCMAAgAyTWFjaW50b3NoIEhEOlVzZXJzOgBlbGVuYXRoZWRoZWw6AC5UcmFzaDoAaXNpcy5iaWIADgASAAgAaQBzAGkAcwAuAGIAaQBiAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIAIlVzZXJzL2VsZW5hdGhlZGhlbC8uVHJhc2gvaXNpcy5iaWIAEwABLwAAFQACABP//wAAgAbSGxwdHlokY2xhc3NuYW1lWCRjbGFzc2VzXU5TTXV0YWJsZURhdGGjHR8gVk5TRGF0YVhOU09iamVjdNIbHCIjXE5TRGljdGlvbmFyeaIiIF8QD05TS2V5ZWRBcmNoaXZlctEmJ1Ryb290gAEACAARABoAIwAtADIANwBAAEYATQBVAGAAZwBqAGwAbgBxAHMAdQB3AIQAjgCpAK4AtgIiAiQCKQI0Aj0CSwJPAlYCXwJkAnECdAKGAokCjgAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKQ},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/159303}}

@article{miller16gx340,
	Abstract = {We present a spectral analysis of a brief Chandra /HETG observation of the neutron star low-mass X-ray binary GX 340+0. The high-resolution spectrum reveals evidence of ionized absorption in the Fe K band. The strongest feature, an absorption line at approximately 6.9 keV, is required at the 5 σ level of confidence via an F -test. Photoionization modeling with XSTAR grids suggests that the line is the most prominent part of a disk wind with an apparent outflow speed of v = 0.04 c . This interpretation is preferred at the 4 σ level over a scenario in which the line is H-like Fe xxvi at a modest redshift. The wind may achieve this speed owing to its relatively low ionization, enabling driving by radiation pressure on lines; in this sense, the wind in GX 340+0 may be the stellar-mass equivalent of the flows in broad absorption line quasars. If the gas has a unity volume filling factor, the mass ouflow rate in the wind is over 10 −5 M ⊙ yr −1 , and the kinetic power is nearly 10 39 erg s −1 (or, 5--6 times the radiative Eddington limit for a neutron star). However, geometrical considerations---including a small volume filling factor and low covering factor---likely greatly reduce these values.},
	Author = {J. M. Miller and J. Raymond and E. Cackett and V. Grinberg and M. Nowak},
	Date-Added = {2016-10-06 20:04:50 +0000},
	Date-Modified = {2016-10-06 20:04:59 +0000},
	Journal = {The Astrophysical Journal Letters},
	Number = {1},
	Pages = {L18},
	Title = {An Ultra-fast X-Ray Disk Wind in the Neutron Star Binary GX 340+0},
	Url = {http://stacks.iop.org/2041-8205/822/i=1/a=L18},
	Volume = {822},
	Year = {2016},
	Bdsk-Url-1 = {http://stacks.iop.org/2041-8205/822/i=1/a=L18}}

@article{progakallman02,
	Abstract = {X-ray heating of the photosphere of an accretion disk is a possible mechanism to produce strong, broad UV emission lines in low-mass X-ray binaries (LMXBs). However, detailed photoionization calculations show that this mechanism fails to produce sufficient emission measure at suitable ionization and optical depth. We present the results of hydrodynamical calculations of the disk photosphere irradiated by strong X-rays. We attempt to determine whether LMXBs can harbor significant UV-driven disk winds despite the effects of X-ray ionization. Such winds would be a likely candidate for the site of emission of UV lines and may better explain the observations than the X-ray-heated disk photosphere. We find that the local disk radiation cannot launch a wind from the disk because of strong ionizing radiation from the central object. Unphysically high X-ray opacities would be required to shield the UV-emitting disk and allow the line force to drive a disk wind. However, the same X-ray radiation that inhibits line driving heats the disk and can produce a hot bipolar wind or corona above the disk. Our calculations are generally consistent with past work on the dynamics of coronae and winds from accretion disks in LMXBs. Additionally, our results are consistent with the UV observations of LMXB that show no obvious spectral features associated with strong and fast disk winds. To assess the impact of X-ray heating on driving of a disk wind by the line force in any system with an accretion disk, we derive analytic formulae. In particular, we compare results of line-driven disk wind models for accretion disks in LMXBs and active galactic nuclei. The latter show spectral features associated with a strong and fast disk wind, the wind that has been successfully modeled by Proga, Stone, & Kallman. The key parameter determining the role of the line force is not merely the presence of the luminous UV zone in the disk and the presence of the X-rays but also the distance of this UV zone from the center. The closer the UV zone to the center, the stronger the line force and subsequently the denser the disk wind launched by the line force. The density of the disk wind critically determines whether the wind will stay in a lower ionization state in the presence of the X-ray radiation and be further accelerated by the line force to supersonic velocities.},
	Author = {Daniel Proga and Timothy R. Kallman},
	Date-Added = {2016-10-06 19:31:40 +0000},
	Date-Modified = {2016-10-06 19:31:48 +0000},
	Journal = {The Astrophysical Journal},
	Number = {1},
	Pages = {455},
	Title = {On the Role of the Ultraviolet and X-Ray Radiation in Driving a Disk Wind in X-Ray Binaries},
	Url = {http://stacks.iop.org/0004-637X/565/i=1/a=455},
	Volume = {565},
	Year = {2002},
	Bdsk-Url-1 = {http://stacks.iop.org/0004-637X/565/i=1/a=455}}

@article{woods96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...461..767W},
	Author = {{Woods}, D.~T. and {Klein}, R.~I. and {Castor}, J.~I. and {McKee}, C.~F. and {Bell}, J.~B.},
	Date-Added = {2016-10-06 19:27:48 +0000},
	Date-Modified = {2016-10-06 19:27:52 +0000},
	Doi = {10.1086/177101},
	Journal = {\apj},
	Keywords = {ACCRETION, ACCRETION DISKS, GALAXIES: ACTIVE, HYDRODYNAMICS, STARS: CORONAE, X-RAYS: GALAXIES, X-RAYS: STARS},
	Month = apr,
	Pages = {767},
	Title = {{X-Ray--heated Coronae and Winds from Accretion Disks: Time-dependent Two-dimensional Hydrodynamics with Adaptive Mesh Refinement}},
	Volume = 461,
	Year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/177101}}

@article{neilsen12,
	Abstract = {During its 2005 outburst, GRO J1655-40 was observed twice with the Chandra High Energy Transmission Grating Spectrometer; the second observation revealed a spectrum rich with ionized absorption lines from elements ranging from O to Ni, indicative of an outflow too dense and too ionized to be driven by radiation or thermal pressure. To date, this spectrum is the only definitive evidence of an ionized wind driven off the accretion disk by magnetic processes in a black hole X-ray binary. Here we present our detailed spectral analysis of the first Chandra observation, nearly three weeks earlier, in which the only signature of the wind is the Fe XXVI absorption line. Comparing the broadband X-ray spectra via photoionization models, we argue that the differences in the Chandra spectra cannot possibly be explained by the changes in the ionizing spectrum, which implies that the properties of the wind cannot be constant throughout the outburst. We explore physical scenarios for the changes in the wind, which we suggest may begin as a hybrid MHD/thermal wind, but evolves over the course of weeks into two distinct outflows with different properties. We discuss the implications of our results for the links between the state of the accretion flow and the presence of transient disk winds.},
	Author = {Joseph Neilsen and Jeroen Homan},
	Date-Added = {2016-10-06 15:41:05 +0000},
	Date-Modified = {2016-10-06 15:41:32 +0000},
	Journal = {The Astrophysical Journal},
	Number = {1},
	Pages = {27},
	Title = {A Hybrid Magnetically/Thermally Driven Wind in the Black Hole GRO J1655--40?},
	Url = {http://stacks.iop.org/0004-637X/750/i=1/a=27},
	Volume = {750},
	Year = {2012},
	Bdsk-Url-1 = {http://stacks.iop.org/0004-637X/750/i=1/a=27}}

@article{lee01,
	Abstract = {The time-averaged 30 ks Chandra AO1 High Energy Transmission Grating Spectrometer observation of the microquasar GRS 1915+105 in the low hard state reveals for the first time in this source neutral K absorption edges from iron, silicon, magnesium, and sulphur. Ionized resonance ( r ) absorption from H- and He-like species of Fe ( XXV , XXVI ) and possibly Ca XX are also seen as well as possible emission from neutral Fe Kα and ionized Fe XXV (forbidden or the resonance emission component of a P Cygni profile). We report the tentative detection of the first astrophysical signature of X-ray absorption fine structure in the photoelectric edge of Si (and possibly Fe and Mg) attributed to material in grains. The large column densities measured from the neutral edges reveal anomalous Si and Fe abundances and illustrate the importance of high-resolution X-ray measurements for assessing material that surrounds bright X-ray sources, especially if depletion onto grains plays a prominent role. Scenarios for which the anomalous abundances can be attributed to surrounding cold material associated with GRS 1915+105 and/or for which the enrichment may signify either a highly unusual supernova/hypernova or external supernova activity local to the binary are discussed. We attribute the ionized features to a hot disk, disk wind, or corona environment. Based on H- and He-like Fe ( XXV , XXVI ), we estimate constraints on the ionization parameter (log ξ ##IMG## [http://ej.iop.org/icons/Entities/gtrsim.gif] {gtrsim} 4.15), temperature ( T > 2.4 × 10 6 K), and hydrogen equivalent number density ( n ##IMG## [http://ej.iop.org/icons/Entities/gtrsim.gif] {gtrsim} 10 12 cm -3 ) for this region. Variability studies with the simultaneous RXTE data show that the light-curve count rate tracks the changes in the disk blackbody as well as the power-law flux, with the most significant variations observed in the former. The Chandra data show spectral changes that also track the behavior of the light curve and may point to changes in both the ionizing flux and density of the absorber. A 3.69 Hz quasi-periodic oscillation and weak first harmonic are seen in the RXTE data.},
	Author = {Julia C. Lee and Christopher S. Reynolds and Ronald Remillard and Norbert S. Schulz and Eric G. Blackman and Andrew C. Fabian},
	Date-Added = {2016-10-06 15:37:50 +0000},
	Date-Modified = {2016-10-06 15:37:57 +0000},
	Journal = {The Astrophysical Journal},
	Number = {2},
	Pages = {1102},
	Title = {High-Resolution Chandra HETGS and Rossi X-Ray Timing Explorer Observations of GRS 1915+105: A Hot Disk Atmosphere and Cold Gas Enriched in Iron and Silicon},
	Url = {http://stacks.iop.org/0004-637X/567/i=2/a=1102},
	Volume = {567},
	Year = {2002},
	Bdsk-Url-1 = {http://stacks.iop.org/0004-637X/567/i=2/a=1102}}

@article{chakravorty2013,
	Abstract = {We present a systematic theory-motivated study of the thermodynamic stability condition as an explanation for the observed accretion disc wind signatures in different states of low-mass black hole binaries (BHB). The variability in observed ions is conventionally explained either by variations in the driving mechanisms or by the changes in the ionizing flux or due to density effects, whilst thermodynamic stability considerations have been largely ignored. It would appear that the observability of particular ions in different BHB states can be accounted for through simple thermodynamic considerations in the static limit. Our calculations predict that in the disc-dominated soft thermal and intermediate states, the wind should be thermodynamically stable and hence observable. On the other hand, in the power-law-dominated spectrally hard state the wind is found to be thermodynamically unstable for a certain range of 3.55 ≤ log?? ≤ 4.20. In the spectrally hard state, a large number of the He-like and H-like ions (including e.g. Fe?xxv, Ar?xviii and S?xv) have peak ion fractions in the unstable ionization parameter (?) range, making these ions undetectable. Our theoretical predictions have clear corroboration in the literature reporting differences in wind ion observability as the BHBs transition through the accretion states While this effect may not be the only one responsible for the observed gradient in the wind properties as a function of the accretion state in BHBs, it is clear that its inclusion in the calculations is crucial for understanding the link between the environment of the compact object and its accretion processes.},
	Author = {Chakravorty, Susmita and Lee, Julia C. and Neilsen, Joseph},
	Date-Added = {2016-10-03 21:16:05 +0000},
	Date-Modified = {2016-10-03 21:16:14 +0000},
	Doi = {10.1093/mnras/stt1593},
	Eprint = {http://mnras.oxfordjournals.org/content/436/1/560.full.pdf+html},
	Journal = {Monthly Notices of the Royal Astronomical Society},
	Number = {1},
	Pages = {560-569},
	Title = {The effects of thermodynamic stability on wind properties in different low-mass black hole binary states},
	Url = {http://mnras.oxfordjournals.org/content/436/1/560.abstract},
	Volume = {436},
	Year = {2013},
	Bdsk-Url-1 = {http://mnras.oxfordjournals.org/content/436/1/560.abstract},
	Bdsk-Url-2 = {http://dx.doi.org/10.1093/mnras/stt1593}}

@article{shields86,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1986ApJ...306...90S},
	Author = {{Shields}, G.~A. and {McKee}, C.~F. and {Lin}, D.~N.~C. and {Begelman}, M.~C.},
	Date-Added = {2016-09-30 18:55:32 +0000},
	Date-Modified = {2016-09-30 18:55:41 +0000},
	Doi = {10.1086/164322},
	Journal = {\apj},
	Keywords = {Accretion Disks, Compton Effect, Magnetohydrodynamic Stability, Plasma Heating, Stellar Oscillations, Stellar Winds, Active Galactic Nuclei, Computational Astrophysics, Plasma Oscillations, Stellar Coronas, Stellar Mass Accretion, Stellar Mass Ejection, X Ray Binaries},
	Month = jul,
	Pages = {90-106},
	Title = {{Compton-heated winds and coronae above accretion disks. II - Instability and oscillations}},
	Volume = 306,
	Year = 1986,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/164322}}

@article{begel83,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1983ApJ...271...89B},
	Author = {{Begelman}, M.~C. and {McKee}, C.~F.},
	Date-Added = {2016-09-30 18:53:57 +0000},
	Date-Modified = {2016-09-30 18:54:03 +0000},
	Doi = {10.1086/161179},
	Journal = {\apj},
	Keywords = {Accretion Disks, Binary Stars, Compton Effect, Radiative Transfer, Stellar Winds, X Ray Sources, Galactic Nuclei, Incident Radiation, Quasars, Seyfert Galaxies, Stellar Coronas, Stellar Mass Accretion, X Ray Binaries},
	Month = aug,
	Pages = {89-112},
	Title = {{Compton heated winds and coronae above accretion disks. II Radiative transfer and observable consequences}},
	Volume = 271,
	Year = 1983,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/161179}}

@article{miller06H1743,
	Abstract = {We observed the bright phase of the 2003 outburst of the Galactic black hole candidate H1743-322 in X-rays simultaneously with Chandra and RXTE on four occasions. The Chandra HETGS spectra reveal narrow, variable (He-like) Fe XXV and (H-like) Fe XXVI resonance absorption lines. In the first observation, the Fe XXVI line has a FWHM of 1800 $\pm$ 400 km s -1 and a blueshift of 700 $\pm$ 200 km s -1 , suggesting that the highly ionized medium is an outflow. Moreover, the Fe XXV line is observed to vary significantly on a timescale of a few hundred seconds in the first observation, which corresponds to the Keplerian orbital period at approximately 10 4 r g (where r g = GM / c 2 ). Our models for the absorption geometry suggest that a combination of changing ionizing flux and geometric effects are required to account for the large changes in line flux observed between observations and that the absorption likely occurs at a radius between 10 2 r g and 10 4 r g for a 10 M ☉ black hole. We suggest that the absorption occurs in an inhomogeneous accretion disk wind. If the wind in H1743-322 has unity filling factor, the highest implied mass outflow rate is 5% of the Eddington mass accretion rate. The observed wind may be a hotter, more ionized version of the Seyfert-like, outflowing warm absorber geometries recently found in the Galactic black holes GX 339-4 and XTE J1650-500. We discuss these findings in the context of ionized Fe absorption lines found in the spectra of other Galactic sources, and connections to warm absorbers, winds and jets in other accreting systems.},
	Author = {J. M. Miller and J. Raymond and J. Homan and A. C. Fabian and D. Steeghs and R. Wijnands and M. Rupen and P. Charles and M. van der Klis and W. H. G. Lewin},
	Date-Added = {2016-09-27 17:28:55 +0000},
	Date-Modified = {2016-09-27 17:29:13 +0000},
	Journal = {The Astrophysical Journal},
	Number = {1},
	Pages = {394},
	Title = {Simultaneous Chandra and RXTE Spectroscopy of the Microquasar H1743--322: Clues to Disk Wind and Jet Formation from a Variable Ionized Outflow},
	Url = {http://stacks.iop.org/0004-637X/646/i=1/a=394},
	Volume = {646},
	Year = {2006},
	Bdsk-Url-1 = {http://stacks.iop.org/0004-637X/646/i=1/a=394}}

@article{neilsenlee09,
	Annote = {10.1038/nature07680},
	Author = {Neilsen, Joseph and Lee, Julia C.},
	Date = {2009/03/26/print},
	Date-Added = {2016-09-27 17:10:34 +0000},
	Date-Modified = {2016-09-27 17:10:42 +0000},
	Day = {26},
	Isbn = {0028-0836},
	Journal = {Nature},
	L3 = {http://www.nature.com/nature/journal/v458/n7237/suppinfo/nature07680_S1.html},
	M3 = {10.1038/nature07680},
	Month = {03},
	Number = {7237},
	Pages = {481--484},
	Publisher = {Macmillan Publishers Limited. All rights reserved},
	Title = {Accretion disk winds as the jet suppression mechanism in the microquasar GRS 1915+105},
	Ty = {JOUR},
	Url = {http://dx.doi.org/10.1038/nature07680},
	Volume = {458},
	Year = {2009},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature07680}}

@article{ponti14,
	Abstract = {High-resolution X-ray spectra of accreting stellar-mass black holes reveal the presence of accretion disc winds, traced by high-ionization Fe K lines. These winds appear to have an equatorial geometry and to be observed only during disc-dominated states in which the radio jet is absent. Accreting neutron star systems also show equatorial high-ionization absorbers. However, the presence of any correlation with the accretion state has not been previously tested. We have studied EXO 0748-676, a transient neutron star system, for which we can reliably determine the accretion state, in order to investigate the Fe K absorption/accretion state/jet connection. Not one of 20 X-ray spectra obtained in the hard state revealed any significant Fe K absorption line. However, intense Fe xxv and Fe xxvi (as well as a rarely observed Fe xxiii line plus S xvi; a blend of S xvi and Ar xvii; Ca xx and Ca xix, possibly produced by the same high-ionization material) absorption lines (${\rm EW}_{\rm Fe\,{\small XXIII-XXV}}=31\pm 3$, ${\rm EW}_{\rm Fe\,{\small XXVI}}=8\pm 3$ eV) are clearly detected during the only soft-state observation. This suggests that the connection between Fe K absorption and states (and anticorrelation between the presence of Fe K absorption and jets) is also valid for EXO 0748-676 and therefore it is not a unique property of black hole systems but a more general characteristic of accreting sources.},
	Author = {Ponti, Gabriele and Mu{\~n}oz-Darias, Teodoro and Fender, Robert P.},
	Date-Added = {2016-09-27 16:49:15 +0000},
	Date-Modified = {2016-09-27 16:49:27 +0000},
	Doi = {10.1093/mnras/stu1742},
	Eprint = {http://mnras.oxfordjournals.org/content/444/2/1829.full.pdf+html},
	Journal = {Monthly Notices of the Royal Astronomical Society},
	Number = {2},
	Pages = {1829-1834},
	Title = {A connection between accretion state and Fe K absorption in an accreting neutron star: black hole-like soft-state winds?},
	Url = {http://mnras.oxfordjournals.org/content/444/2/1829.abstract},
	Volume = {444},
	Year = {2014},
	Bdsk-Url-1 = {http://mnras.oxfordjournals.org/content/444/2/1829.abstract},
	Bdsk-Url-2 = {http://dx.doi.org/10.1093/mnras/stu1742}}

@article{higproga15,
	Abstract = {X-ray and UV line emission in X-ray binaries (XRBs) can be accounted for by a hot corona. Such a corona forms through irradiation of the outer disk by radiation produced in the inner accretion flow. The same irradiation can produce a strong outflow from the disk at sufficiently large radii. Outflowing gas has been recently detected in several XRBs via blueshifted absorption lines. However, the causal connection between winds produced by irradiation and the blueshifted absorption lines is problematic, particularly in the case of GRO J1655--40. Observations of this source imply wind densities about two orders of magnitude higher than theoretically predicted. This discrepancy does not mean that these ``thermal disk winds'' cannot explain blueshifted absorption in other systems, nor that they are unimportant as a sink of matter. Motivated by the inevitability of thermal disk winds and wealth of data taken with current observatories such as Chandra , XMM-Newton , and Suzaku , as well as the future AstroH mission, we decided to investigate the requirements to produce very dense winds. Using physical arguments, hydrodynamical simulations, and absorption-line calculations, we found that modification of the heating and cooling rates by a factor of a few results in an increase of the wind density of up to an order of magnitude and the wind velocity by a factor of about two. Therefore, the mass-loss rate from the disk can be one, if not even two, orders of magnitude higher than the accretion rate onto the central object. Such a high mass-loss rate is expected to destabilize the disk and perhaps provides a mechanism for state change.},
	Author = {Nick Higginbottom and Daniel Proga},
	Date-Added = {2016-09-27 16:40:43 +0000},
	Date-Modified = {2016-09-27 16:40:55 +0000},
	Journal = {The Astrophysical Journal},
	Number = {1},
	Pages = {107},
	Title = {Coronae and Winds from Irradiated Disks in X-Ray Binaries},
	Url = {http://stacks.iop.org/0004-637X/807/i=1/a=107},
	Volume = {807},
	Year = {2015},
	Bdsk-Url-1 = {http://stacks.iop.org/0004-637X/807/i=1/a=107}}

@article{wilmsabund,
	Abstract = {We present an improved model for the absorption of X-rays in the interstellar medium (ISM) intended for use with data from future X-ray missions with larger effective areas and increased energy resolution such as Chandra and the X-Ray Multiple Mirror mission, in the energy range ##IMG## [http://ej.iop.org/icons/Entities/gtrsim.gif] {gtrsim} 100 eV. Compared with previous work, our formalism includes recent updates to the photoionization cross section and revised abundances of the interstellar medium, as well as a treatment of interstellar grains and the H 2 molecule. We review the theoretical and observational motivations behind these updates and provide a subroutine for the X-ray spectral analysis program XSPEC that incorporates our model.},
	Author = {J. Wilms and A. Allen and R. McCray},
	Date-Added = {2016-08-01 00:53:56 +0000},
	Date-Modified = {2016-08-01 00:54:12 +0000},
	Isbn = {0004-637X},
	Journal = {The Astrophysical Journal},
	Number = {2},
	Sp = {914},
	Title = {On the Absorption of X-Rays in the Interstellar Medium},
	Ty = {JOUR},
	Url = {http://stacks.iop.org/0004-637X/542/i=2/a=914},
	Volume = {542},
	Year = {2000},
	Bdsk-Url-1 = {http://stacks.iop.org/0004-637X/542/i=2/a=914}}

@article{juettchakshifts,
	Abstract = {We present the high-resolution Chandra X-Ray Observatory persistent (nondip) spectrum of 4U 1916-05, which revealed narrow absorption lines from hydrogenic neon, magnesium, silicon, and sulfur, in addition to the previous identified hydrogenic and helium-like iron absorption lines. This makes 4U 1916-05 only the second of the classical X-ray dipper systems to show narrow absorption lines from elements other than iron. We propose two possible explanations for the small measured line widths ( ##IMG## [http://ej.iop.org/icons/Entities/lesssim.gif] {lesssim} 500-2000 km s -1 ), compared to the expected Keplerian velocities (>1000 km s -1 ) of the accretion disk in this 50 minute orbital period system, and lack of wavelength shifts ( ##IMG## [http://ej.iop.org/icons/Entities/lesssim.gif] {lesssim} 250 km s -1 ). First, the ionized absorber may be stationary. Alternatively, the line properties may measure the relative size of the emission region. From this hypothesis, we find that the emission region is constrained to be ##IMG## [http://ej.iop.org/icons/Entities/lesssim.gif] {lesssim} 0.25 times the radial extent of the absorber. Our results also imply that the ionized absorber spans a range of ionization parameters.},
	Author = {Adrienne M. Juett and Deepto Chakrabarty},
	Date-Added = {2016-07-31 20:22:43 +0000},
	Date-Modified = {2016-07-31 20:22:54 +0000},
	Isbn = {0004-637X},
	Journal = {The Astrophysical Journal},
	Number = {1},
	Sp = {493},
	Title = {Detection of Highly Ionized Metal Absorption Lines in the Ultracompact X-Ray Dipper 4U 1916--05},
	Ty = {JOUR},
	Url = {http://stacks.iop.org/0004-637X/646/i=1/a=493},
	Volume = {646},
	Year = {2006},
	Bdsk-Url-1 = {http://stacks.iop.org/0004-637X/646/i=1/a=493}}

@article{miller15multabs,
	Abstract = {We present an analysis of ionized X-ray disk winds found in the Fe K band of four stellar-mass black holes observed with Chandra , including 4U 1630−47, GRO J1655−40, H 1743−322, and GRS 1915+105. High-resolution photoionization grids were generated in order to model the data. Third-order gratings spectra were used to resolve complex absorption profiles into atomic effects and multiple velocity components. The Fe xxv line is found to be shaped by contributions from the intercombination line (in absorption), and the Fe xxvi line is detected as a spin--orbit doublet. The data require 2--3 absorption zones, depending on the source. The fastest components have velocities approaching or exceeding ##IMG## [http://ej.iop.org/images/0004-637X/814/2/87/apj520930ieqn1.gif] {$0.01c,$} increasing mass outflow rates and wind kinetic power by orders of magnitude over prior single-zone models. The first-order spectra require re-emission from the wind, broadened by a degree that is loosely consistent with Keplerian orbital velocities at the photoionization radius. This suggests that disk winds are rotating with the orbital velocity of the underlying disk, and provides a new means of estimating launching radii---crucial to understanding wind driving mechanisms. Some aspects of the wind velocities and radii correspond well to the broad-line region in active galactic nuclei (AGNs), suggesting a physical connection. We discuss these results in terms of prevalent models for disk wind production and disk accretion itself, and implications for massive black holes in AGNs.},
	Author = {J. M. Miller and A. C. Fabian and J. Kaastra and T. Kallman and A. L. King and D. Proga and J. Raymond and C. S. Reynolds},
	Date-Added = {2016-07-31 20:17:49 +0000},
	Date-Modified = {2018-06-22 00:37:46 +0000},
	Isbn = {0004-637X},
	Journal = {The Astrophysical Journal},
	Number = {2},
	Pages = {87},
	Title = {Powerful, Rotating Disk Winds from Stellar-mass Black Holes},
	Ty = {JOUR},
	Url = {http://stacks.iop.org/0004-637X/814/i=2/a=87},
	Volume = {814},
	Year = {2015},
	Bdsk-Url-1 = {http://stacks.iop.org/0004-637X/814/i=2/a=87}}

@article{miller16,
	Abstract = {We report on a 120 ks Chandra /HETG spectrum of the black hole GRS 1915+105. The observation was made during an extended and bright soft state in 2015 June. An extremely rich disk wind absorption spectrum is detected, similar to that observed at lower sensitivity in 2007. The very high resolution of the third-order spectrum reveals four components to the disk wind in the Fe K band alone; the fastest has a blueshift of ##IMG## [http://ej.iop.org/images/2041-8205/821/1/L9/apjl523217ieqn1.gif] {$v=0.03c$} . Broadened re-emission from the wind is also detected in the first-order spectrum, giving rise to clear accretion disk P Cygni profiles. Dynamical modeling of the re-emission spectrum gives wind launching radii of ##IMG## [http://ej.iop.org/images/2041-8205/821/1/L9/apjl523217ieqn2.gif] {$r\simeq {10}^{2-4}\;\mathrm{GM}/{{\rm{c}}}^{2}$} . Wind density values of ##IMG## [http://ej.iop.org/images/2041-8205/821/1/L9/apjl523217ieqn3.gif] {$n\simeq {10}^{13-16}\;{{\rm{cm}}}^{-3}$} are then required by the ionization parameter formalism. The small launching radii, high density values, and inferred high mass outflow rates signal a role for magnetic driving. With simple, reasonable assumptions, the wind properties constrain the magnitude of the emergent magnetic field to be ##IMG## [http://ej.iop.org/images/2041-8205/821/1/L9/apjl523217ieqn4.gif] {$B\simeq {10}^{3-4}$} G if the wind is driven via magnetohydrodynamic (MHD) pressure from within the disk and ##IMG## [http://ej.iop.org/images/2041-8205/821/1/L9/apjl523217ieqn5.gif] {$B\simeq {10}^{4-5}$} G if the wind is driven by magnetocentrifugal acceleration. The MHD estimates are below upper limits predicted by the canonical α -disk model. We discuss these results in terms of fundamental disk physics and black hole accretion modes.},
	Author = {J. M. Miller and J. Raymond and A. C. Fabian and E. Gallo and J. Kaastra and T. Kallman and A. L. King and D. Proga and C. S. Reynolds and A. Zoghbi},
	Date-Added = {2016-07-31 19:56:08 +0000},
	Date-Modified = {2018-06-22 00:38:11 +0000},
	Isbn = {2041-8205},
	Journal = {The Astrophysical Journal Letters},
	Number = {1},
	Pages = {L9},
	Title = {The Accretion Disk Wind in the Black Hole GRS 1915+105},
	Ty = {JOUR},
	Url = {http://stacks.iop.org/2041-8205/821/i=1/a=L9},
	Volume = {821},
	Year = {2016},
	Bdsk-Url-1 = {http://stacks.iop.org/2041-8205/821/i=1/a=L9}}

@article{kallman09,
	Abstract = {The spectrum from the black hole X-ray transient GRO J1655-40 obtained using the Chandra High Energy Transmission Grating in 2005 is notable as a laboratory for the study of warm absorbers, and for the presence of many lines from odd- Z elements between Na and Co (and Ti and Cr) not previously observed in X-rays. We present synthetic spectral models which can be used to constrain these element abundances and other parameters describing the outflow from the warm absorber in this object. We present results of fitting to the spectrum using various tools and techniques, including automated line fitting, phenomenological models, and photoionization modeling. We show that the behavior of the curves of growth of lines from H-like and Li-like ions indicate that the lines are either saturated or affected by filling-in from scattered or a partially covered continuum source. We confirm the conclusion of previous work by Miller et al., which shows that the ionization conditions are not consistent with wind driving due to thermal expansion. The spectrum provides the opportunity to measure abundances for several elements not typically observable in the X-ray band. These show a pattern of enhancement for iron peak elements, and solar or subsolar values for elements lighter than calcium. Models show that this is consistent with enrichment by a core-collapse supernova. We discuss the implications of these values for the evolutionary history of this system.},
	Author = {T. R. Kallman and M. A. Bautista and Stephane Goriely and Claudio Mendoza and Jon M. Miller and Patrick Palmeri and Pascal Quinet and John Raymond},
	Date-Added = {2016-07-31 19:43:15 +0000},
	Date-Modified = {2018-06-22 00:36:17 +0000},
	Isbn = {0004-637X},
	Journal = {The Astrophysical Journal},
	Number = {2},
	Pages = {865},
	Title = {Spectrum Synthesis Modeling of the X-Ray Spectrum of GRO J1655-40 Taken During the 2005 Outburst},
	Ty = {JOUR},
	Url = {http://stacks.iop.org/0004-637X/701/i=2/a=865},
	Volume = {701},
	Year = {2009},
	Bdsk-Url-1 = {http://stacks.iop.org/0004-637X/701/i=2/a=865}}

@article{miller06,
	Annote = {10.1038/nature04912},
	Author = {Miller, Jon M. and Raymond, John and Fabian, Andy and Steeghs, Danny and Homan, Jeroen and Reynolds, Chris and van der Klis, Michiel and Wijnands, Rudy},
	Date = {2006/06/22/print},
	Date-Added = {2016-07-31 19:41:11 +0000},
	Date-Modified = {2016-07-31 19:41:27 +0000},
	Day = {22},
	Isbn = {0028-0836},
	Journal = {Nature},
	L3 = {http://www.nature.com/nature/journal/v441/n7096/suppinfo/nature04912_S1.html},
	M3 = {10.1038/nature04912},
	Month = {06},
	Number = {7096},
	Pages = {953--955},
	Title = {The magnetic nature of disk accretion onto black holes},
	Ty = {JOUR},
	Url = {http://dx.doi.org/10.1038/nature04912},
	Volume = {441},
	Year = {2006},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUGJCVYJHZlcnNpb25YJG9iamVjdHNZJGFyY2hpdmVyVCR0b3ASAAGGoKgHCBMUFRYaIVUkbnVsbNMJCgsMDxJXTlMua2V5c1pOUy5vYmplY3RzViRjbGFzc6INDoACgAOiEBGABIAFgAdccmVsYXRpdmVQYXRoWWFsaWFzRGF0YV8QIi4uLy4uLy4uLy5UcmFzaC9taWxsZXIxNl9neDM0MC5iaWLSFwsYGVdOUy5kYXRhTxEBkAAAAAABkAACAAAMTWFjaW50b3NoIEhEAAAAAAAAAAAAAAAAAAAAyrj/FEgrAAA7A7gJEm1pbGxlcjE2X2d4MzQwLmJpYgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAADrw5tLUHCaNAAAAAAAAAAAAAwACAAAJIAAAAAAAAAAAAAAAAAAAAAYuVHJhc2gAEAAIAADKuTdUAAAAEQAIAADUHF7NAAAAAQAMOwO4CQAFHuoAAMAjAAIAPE1hY2ludG9zaCBIRDpVc2VyczoAZWxlbmF0aGVkaGVsOgAuVHJhc2g6AG1pbGxlcjE2X2d4MzQwLmJpYgAOACYAEgBtAGkAbABsAGUAcgAxADYAXwBnAHgAMwA0ADAALgBiAGkAYgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASACxVc2Vycy9lbGVuYXRoZWRoZWwvLlRyYXNoL21pbGxlcjE2X2d4MzQwLmJpYgATAAEvAAAVAAIAE///AACABtIbHB0eWiRjbGFzc25hbWVYJGNsYXNzZXNdTlNNdXRhYmxlRGF0YaMdHyBWTlNEYXRhWE5TT2JqZWN00hscIiNcTlNEaWN0aW9uYXJ5oiIgXxAPTlNLZXllZEFyY2hpdmVy0SYnVHJvb3SAAQAIABEAGgAjAC0AMgA3AEAARgBNAFUAYABnAGoAbABuAHEAcwB1AHcAhACOALMAuADAAlQCVgJbAmYCbwJ9AoECiAKRApYCowKmArgCuwLAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAsI=},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature04912}}

@article{ueda2004,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...609..325U},
	Author = {{Ueda}, Y. and {Murakami}, H. and {Yamaoka}, K. and {Dotani}, T. and {Ebisawa}, K.},
	Doi = {10.1086/420973},
	Journal = {\apj},
	Keywords = {Stars: Individual: Alphanumeric: GX 13+1, X-Rays: Binaries, X-Rays: Stars},
	Month = jul,
	Pages = {325-334},
	Title = {{Chandra High-Resolution Spectroscopy of the Absorption-Line Features in the Low-Mass X-Ray Binary GX 13+1}},
	Volume = 609,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/420973}}

@article{ueda2001,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...556L..87U},
	Author = {{Ueda}, Y. and {Asai}, K. and {Yamaoka}, K. and {Dotani}, T. and {Inoue}, H.},
	Doi = {10.1086/323007},
	Journal = {\apjl},
	Keywords = {Stars: Individual: Alphanumeric: GX 13+1, X-Rays: Stars},
	Month = aug,
	Pages = {L87-L90},
	Title = {{Discovery of an Iron K Absorption Line in the Low-Mass X-Ray Binary GX 13+1}},
	Volume = 556,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/323007}}

@article{pontibh12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.422L..11P},
	Archiveprefix = {arXiv},
	Author = {{Ponti}, G. and {Fender}, R.~P. and {Begelman}, M.~C. and {Dunn}, R.~J.~H. and {Neilsen}, J. and {Coriat}, M.},
	Doi = {10.1111/j.1745-3933.2012.01224.x},
	Eprint = {1201.4172},
	Journal = {\mnras},
	Keywords = {accretion, accretion disc, blackhole physics, methods: observational, techniques: spectroscopic, quasars: absorption lines, X-rays: binaries},
	Month = may,
	Pages = {L11},
	Primaryclass = {astro-ph.HE},
	Title = {{Ubiquitous equatorial accretion disc winds in black hole soft states}},
	Volume = 422,
	Year = 2012,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUGJCVYJHZlcnNpb25YJG9iamVjdHNZJGFyY2hpdmVyVCR0b3ASAAGGoKgHCBMUFRYaIVUkbnVsbNMJCgsMDxJXTlMua2V5c1pOUy5vYmplY3RzViRjbGFzc6INDoACgAOiEBGABIAFgAdccmVsYXRpdmVQYXRoWWFsaWFzRGF0YV8QMy4uL3BhcGVyL2JpYl9jaXRhdGlvbnMvYmlidGV4LWNpdGF0aW9uc19wb250aTE0LmJpYtIXCxgZV05TLmRhdGFPEQHCAAAAAAHCAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAAAAAAAAAAQkQAAf////8cYmlidGV4LWNpdGF0aW9uc19wb250aTE0LmJpYgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAA/////wAAAAAAAAAAAAAAAAABAAMAAAogY3UAAAAAAAAAAAAAAAAADWJpYl9jaXRhdGlvbnMAAAIAVC86VXNlcnM6ZWxlbmF0aGVkaGVsOnJlc2VhcmNoOmd4MTMxOnBhcGVyOmJpYl9jaXRhdGlvbnM6YmlidGV4LWNpdGF0aW9uc19wb250aTE0LmJpYgAOADoAHABiAGkAYgB0AGUAeAAtAGMAaQB0AGEAdABpAG8AbgBzAF8AcABvAG4AdABpADEANAAuAGIAaQBiAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIAUlVzZXJzL2VsZW5hdGhlZGhlbC9yZXNlYXJjaC9neDEzMS9wYXBlci9iaWJfY2l0YXRpb25zL2JpYnRleC1jaXRhdGlvbnNfcG9udGkxNC5iaWIAEwABLwAAFQACABP//wAAgAbSGxwdHlokY2xhc3NuYW1lWCRjbGFzc2VzXU5TTXV0YWJsZURhdGGjHR8gVk5TRGF0YVhOU09iamVjdNIbHCIjXE5TRGljdGlvbmFyeaIiIF8QD05TS2V5ZWRBcmNoaXZlctEmJ1Ryb290gAEACAARABoAIwAtADIANwBAAEYATQBVAGAAZwBqAGwAbgBxAHMAdQB3AIQAjgDEAMkA0QKXApkCngKpArICwALEAssC1ALZAuYC6QL7Av4DAwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAMF},
	Bdsk-File-2 = {YnBsaXN0MDDUAQIDBAUGJCVYJHZlcnNpb25YJG9iamVjdHNZJGFyY2hpdmVyVCR0b3ASAAGGoKgHCBMUFRYaIVUkbnVsbNMJCgsMDxJXTlMua2V5c1pOUy5vYmplY3RzViRjbGFzc6INDoACgAOiEBGABIAFgAdccmVsYXRpdmVQYXRoWWFsaWFzRGF0YV8QJi4uL3BhcGVyL2JpYl9jaXRhdGlvbnMvbmF0dXJlMDc2ODAucmlz0hcLGBlXTlMuZGF0YU8RAZAAAAAAAZAAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAAAAAABCRAAB/////w9uYXR1cmUwNzY4MC5yaXMAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAD/////AAAAAAAAAAAAAAAAAAEAAwAACiBjdQAAAAAAAAAAAAAAAAANYmliX2NpdGF0aW9ucwAAAgBHLzpVc2VyczplbGVuYXRoZWRoZWw6cmVzZWFyY2g6Z3gxMzE6cGFwZXI6YmliX2NpdGF0aW9uczpuYXR1cmUwNzY4MC5yaXMAAA4AIAAPAG4AYQB0AHUAcgBlADAANwA2ADgAMAAuAHIAaQBzAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIARVVzZXJzL2VsZW5hdGhlZGhlbC9yZXNlYXJjaC9neDEzMS9wYXBlci9iaWJfY2l0YXRpb25zL25hdHVyZTA3NjgwLnJpcwAAEwABLwAAFQACABP//wAAgAbSGxwdHlokY2xhc3NuYW1lWCRjbGFzc2VzXU5TTXV0YWJsZURhdGGjHR8gVk5TRGF0YVhOU09iamVjdNIbHCIjXE5TRGljdGlvbmFyeaIiIF8QD05TS2V5ZWRBcmNoaXZlctEmJ1Ryb290gAEACAARABoAIwAtADIANwBAAEYATQBVAGAAZwBqAGwAbgBxAHMAdQB3AIQAjgC3ALwAxAJYAloCXwJqAnMCgQKFAowClQKaAqcCqgK8Ar8CxAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAALG},
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2012.01224.x}}

@article{fleisch85,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1985A%26A...153..106F},
	Author = {{Fleischman}, J.~R.},
	Journal = {\aap},
	Keywords = {X Ray Astronomy, X Ray Sources, Astronomical Maps, Position (Location)},
	Month = dec,
	Pages = {106-108},
	Title = {{Detection of a new X-ray burst source}},
	Volume = 153,
	Year = 1985,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUGJCVYJHZlcnNpb25YJG9iamVjdHNZJGFyY2hpdmVyVCR0b3ASAAGGoKgHCBMUFRYaIVUkbnVsbNMJCgsMDxJXTlMua2V5c1pOUy5vYmplY3RzViRjbGFzc6INDoACgAOiEBGABIAFgAdccmVsYXRpdmVQYXRoWWFsaWFzRGF0YV8QIi4uLy4uLy4uLy5UcmFzaC9taWxsZXIxNl9neDM0MC5iaWLSFwsYGVdOUy5kYXRhTxEBkAAAAAABkAACAAAMTWFjaW50b3NoIEhEAAAAAAAAAAAAAAAAAAAAyrj/FEgrAAA7A7gJEm1pbGxlcjE2X2d4MzQwLmJpYgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAADrw5tLUHCaNAAAAAAAAAAAAAwACAAAJIAAAAAAAAAAAAAAAAAAAAAYuVHJhc2gAEAAIAADKuTdUAAAAEQAIAADUHF7NAAAAAQAMOwO4CQAFHuoAAMAjAAIAPE1hY2ludG9zaCBIRDpVc2VyczoAZWxlbmF0aGVkaGVsOgAuVHJhc2g6AG1pbGxlcjE2X2d4MzQwLmJpYgAOACYAEgBtAGkAbABsAGUAcgAxADYAXwBnAHgAMwA0ADAALgBiAGkAYgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASACxVc2Vycy9lbGVuYXRoZWRoZWwvLlRyYXNoL21pbGxlcjE2X2d4MzQwLmJpYgATAAEvAAAVAAIAE///AACABtIbHB0eWiRjbGFzc25hbWVYJGNsYXNzZXNdTlNNdXRhYmxlRGF0YaMdHyBWTlNEYXRhWE5TT2JqZWN00hscIiNcTlNEaWN0aW9uYXJ5oiIgXxAPTlNLZXllZEFyY2hpdmVy0SYnVHJvb3SAAQAIABEAGgAjAC0AMgA3AEAARgBNAFUAYABnAGoAbABuAHEAcwB1AHcAhACOALMAuADAAlQCVgJbAmYCbwJ9AoECiAKRApYCowKmArgCuwLAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAsI=}}

@article{bandy99,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.306..417B},
	Author = {{Bandyopadhyay}, R.~M. and {Shahbaz}, T. and {Charles}, P.~A. and {Naylor}, T.},
	Doi = {10.1046/j.1365-8711.1999.02547.x},
	Eprint = {astro-ph/9901327},
	Journal = {\mnras},
	Keywords = {ACCRETION, ACCRETION DISCS, BINARIES: CLOSE, BINARIES: SPECTROSCOPIC, INFRARED: STARS, X-RAYS: STARS},
	Month = jun,
	Pages = {417-426},
	Title = {{Infrared spectroscopy of low-mass X-ray binaries - II}},
	Volume = 306,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUGJCVYJHZlcnNpb25YJG9iamVjdHNZJGFyY2hpdmVyVCR0b3ASAAGGoKgHCBMUFRYaIVUkbnVsbNMJCgsMDxJXTlMua2V5c1pOUy5vYmplY3RzViRjbGFzc6INDoACgAOiEBGABIAFgAdccmVsYXRpdmVQYXRoWWFsaWFzRGF0YV8QJC4uLy4uLy4uL0Rvd25sb2Fkcy9JT1BFWFBPUlRfUklTLnJpc9IXCxgZV05TLmRhdGFPEQGWAAAAAAGWAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAAAADKuP8USCsAAAAFHzQRSU9QRVhQT1JUX1JJUy5yaXMAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAOsEZG9PEFaAAAAAAAAAAAAADAAIAAAkgAAAAAAAAAAAAAAAAAAAACURvd25sb2FkcwAAEAAIAADKuTdUAAAAEQAIAADTxE3gAAAAAQAMAAUfNAAFHuoAAMAjAAIAPk1hY2ludG9zaCBIRDpVc2VyczoAZWxlbmF0aGVkaGVsOgBEb3dubG9hZHM6AElPUEVYUE9SVF9SSVMucmlzAA4AJAARAEkATwBQAEUAWABQAE8AUgBUAF8AUgBJAFMALgByAGkAcwAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASAC5Vc2Vycy9lbGVuYXRoZWRoZWwvRG93bmxvYWRzL0lPUEVYUE9SVF9SSVMucmlzABMAAS8AABUAAgAT//8AAIAG0hscHR5aJGNsYXNzbmFtZVgkY2xhc3Nlc11OU011dGFibGVEYXRhox0fIFZOU0RhdGFYTlNPYmplY3TSGxwiI1xOU0RpY3Rpb25hcnmiIiBfEA9OU0tleWVkQXJjaGl2ZXLRJidUcm9vdIABAAgAEQAaACMALQAyADcAQABGAE0AVQBgAGcAagBsAG4AcQBzAHUAdwCEAI4AtQC6AMICXAJeAmMCbgJ3AoUCiQKQApkCngKrAq4CwALDAsgAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACyg==},
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1999.02547.x}}

@article{matsuba95,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1995PASJ...47..575M},
	Author = {{Matsuba}, E. and {Dotani}, T. and {Mitsuda}, K. and {Asai}, K. and {Lewin}, W.~H.~G. and {van Paradijs}, J. and {van der Klis}, M.},
	Journal = {\pasj},
	Keywords = {STARS: INDIVIDUAL (GX 13+1), X-RAYS: BINARIES , X-RAYS: BURSTS, X-RAYS: SOURCES},
	Month = oct,
	Pages = {575-580},
	Title = {{Discovery of X-Ray Bursts from GX 13+1 (4U 1811-17)}},
	Volume = 47,
	Year = 1995}

@article{frid15gx13z,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...809...52F},
	Archiveprefix = {arXiv},
	Author = {{Fridriksson}, J.~K. and {Homan}, J. and {Remillard}, R.~A.},
	Doi = {10.1088/0004-637X/809/1/52},
	Eid = {52},
	Eprint = {1504.00022},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, stars: neutron, X-rays: binaries, X-rays: individual: Cir X-1, Cyg X-2, GX 13+1, XTE J1701{\ndash}462},
	Month = aug,
	Pages = {52},
	Primaryclass = {astro-ph.HE},
	Title = {{Common Patterns in the Evolution between the Luminous Neutron Star Low-Mass X-ray Binary Subclasses}},
	Volume = 809,
	Year = 2015,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUGJCVYJHZlcnNpb25YJG9iamVjdHNZJGFyY2hpdmVyVCR0b3ASAAGGoKgHCBMUFRYaIVUkbnVsbNMJCgsMDxJXTlMua2V5c1pOUy5vYmplY3RzViRjbGFzc6INDoACgAOiEBGABIAFgAdccmVsYXRpdmVQYXRoWWFsaWFzRGF0YV8QJC4uLy4uLy4uL0Rvd25sb2Fkcy9JT1BFWFBPUlRfUklTLnJpc9IXCxgZV05TLmRhdGFPEQGWAAAAAAGWAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAAAADKuP8USCsAAAAFHzQRSU9QRVhQT1JUX1JJUy5yaXMAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAOsEZG9PEFaAAAAAAAAAAAAADAAIAAAkgAAAAAAAAAAAAAAAAAAAACURvd25sb2FkcwAAEAAIAADKuTdUAAAAEQAIAADTxE3gAAAAAQAMAAUfNAAFHuoAAMAjAAIAPk1hY2ludG9zaCBIRDpVc2VyczoAZWxlbmF0aGVkaGVsOgBEb3dubG9hZHM6AElPUEVYUE9SVF9SSVMucmlzAA4AJAARAEkATwBQAEUAWABQAE8AUgBUAF8AUgBJAFMALgByAGkAcwAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASAC5Vc2Vycy9lbGVuYXRoZWRoZWwvRG93bmxvYWRzL0lPUEVYUE9SVF9SSVMucmlzABMAAS8AABUAAgAT//8AAIAG0hscHR5aJGNsYXNzbmFtZVgkY2xhc3Nlc11OU011dGFibGVEYXRhox0fIFZOU0RhdGFYTlNPYmplY3TSGxwiI1xOU0RpY3Rpb25hcnmiIiBfEA9OU0tleWVkQXJjaGl2ZXLRJidUcm9vdIABAAgAEQAaACMALQAyADcAQABGAE0AVQBgAGcAagBsAG4AcQBzAHUAdwCEAI4AtQC6AMICXAJeAmMCbgJ3AoUCiQKQApkCngKrAq4CwALDAsgAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACyg==},
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/809/1/52}}

@article{homan98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...499L..41H},
	Author = {{Homan}, J. and {van der Klis}, M. and {Wijnands}, R. and {Vaughan}, B. and {Kuulkers}, E.},
	Doi = {10.1086/311341},
	Eprint = {astro-ph/9803267},
	Journal = {\apjl},
	Keywords = {ACCRETION, ACCRETION DISKS, STARS: INDIVIDUAL ALPHANUMERIC: GX 13+1, STARS: NEUTRON, X-RAYS: STARS, Accretion, Accretion Disks, Stars: Individual: Alphanumeric: GX 13+1, Stars: Neutron, X-Rays: Stars},
	Month = may,
	Pages = {L41-L44},
	Title = {{Discovery of a 57-69 HZ Quasi-periodic Oscillation in GX 13+1}},
	Volume = 499,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUGJCVYJHZlcnNpb25YJG9iamVjdHNZJGFyY2hpdmVyVCR0b3ASAAGGoKgHCBMUFRYaIVUkbnVsbNMJCgsMDxJXTlMua2V5c1pOUy5vYmplY3RzViRjbGFzc6INDoACgAOiEBGABIAFgAdccmVsYXRpdmVQYXRoWWFsaWFzRGF0YV8QJi4uL3BhcGVyL2JpYl9jaXRhdGlvbnMvbmF0dXJlMDc2ODAucmlz0hcLGBlXTlMuZGF0YU8RAZAAAAAAAZAAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAAAAAABCRAAB/////w9uYXR1cmUwNzY4MC5yaXMAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAD/////AAAAAAAAAAAAAAAAAAEAAwAACiBjdQAAAAAAAAAAAAAAAAANYmliX2NpdGF0aW9ucwAAAgBHLzpVc2VyczplbGVuYXRoZWRoZWw6cmVzZWFyY2g6Z3gxMzE6cGFwZXI6YmliX2NpdGF0aW9uczpuYXR1cmUwNzY4MC5yaXMAAA4AIAAPAG4AYQB0AHUAcgBlADAANwA2ADgAMAAuAHIAaQBzAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIARVVzZXJzL2VsZW5hdGhlZGhlbC9yZXNlYXJjaC9neDEzMS9wYXBlci9iaWJfY2l0YXRpb25zL25hdHVyZTA3NjgwLnJpcwAAEwABLwAAFQACABP//wAAgAbSGxwdHlokY2xhc3NuYW1lWCRjbGFzc2VzXU5TTXV0YWJsZURhdGGjHR8gVk5TRGF0YVhOU09iamVjdNIbHCIjXE5TRGljdGlvbmFyeaIiIF8QD05TS2V5ZWRBcmNoaXZlctEmJ1Ryb290gAEACAARABoAIwAtADIANwBAAEYATQBVAGAAZwBqAGwAbgBxAHMAdQB3AIQAjgC3ALwAxAJYAloCXwJqAnMCgQKFAowClQKaAqcCqgK8Ar8CxAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAALG},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/311341}}

@article{dai14dip,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...564A..62D},
	Archiveprefix = {arXiv},
	Author = {{D'A{\`\i}}, A. and {Iaria}, R. and {Di Salvo}, T. and {Riggio}, A. and {Burderi}, L. and {Robba}, N.~R.},
	Doi = {10.1051/0004-6361/201322044},
	Eid = {A62},
	Eprint = {1403.0071},
	Journal = {\aap},
	Keywords = {X-rays: binaries, radiation mechanisms: general, stars: neutron, atomic processes},
	Month = apr,
	Pages = {A62},
	Primaryclass = {astro-ph.HE},
	Title = {{Chandra X-ray spectroscopy of a clear dip in GX 13+1}},
	Volume = 564,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201322044}}

@article{madej14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.438..145M},
	Archiveprefix = {arXiv},
	Author = {{Madej}, O.~K. and {Jonker}, P.~G. and {D{\'{\i}}az Trigo}, M. and {Mi{\v s}kovi{\v c}ov{\'a}}, I.},
	Doi = {10.1093/mnras/stt2119},
	Eprint = {1311.0874},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, X-rays: binaries, X-rays: individual: GX 13+1},
	Month = feb,
	Pages = {145-155},
	Primaryclass = {astro-ph.HE},
	Title = {{Variable Doppler shifts of the thermal wind absorption lines in low-mass X-ray binaries}},
	Volume = 438,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stt2119}}

@article{sidoli2002,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...385..940S},
	Author = {{Sidoli}, L. and {Parmar}, A.~N. and {Oosterbroek}, T. and {Lumb}, D.},
	Doi = {10.1051/0004-6361:20020192},
	Eprint = {astro-ph/0202077},
	Journal = {\aap},
	Month = apr,
	Pages = {940-946},
	Title = {{Discovery of complex narrow X-ray absorption features from the low-mass X-ray binary GX 13+1 with XMM-Newton}},
	Volume = 385,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20020192}}

@article{dtrigoxmm,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...543A..50D},
	Archiveprefix = {arXiv},
	Author = {{D{\'{\i}}az Trigo}, M. and {Sidoli}, L. and {Boirin}, L. and {Parmar}, A.~N.},
	Doi = {10.1051/0004-6361/201219049},
	Eid = {A50},
	Eprint = {1204.5904},
	Journal = {\aap},
	Keywords = {X-rays: binaries, accretion, accretion disks, X-rays: individuals: GX13+1},
	Month = jul,
	Pages = {A50},
	Primaryclass = {astro-ph.HE},
	Title = {{XMM-Newton observations of GX 13 + 1: correlation between photoionised absorption and broad line emission}},
	Volume = 543,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201219049}}

@article{hasinger89,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...225...79H},
	Author = {{Hasinger}, G. and {van der Klis}, M.},
	Date-Modified = {2018-06-22 00:36:54 +0000},
	Journal = {\aap},
	Keywords = {Neutron Stars, Power Spectra, Stellar Mass Accretion, X Ray Binaries, Color-Color Diagram, Stellar Luminosity, Stellar Spectra},
	Month = nov,
	Pages = {79-96},
	Title = {{Two patterns of correlated X-ray timing and spectral behaviour in low-mass X-ray binaries}},
	Volume = 225,
	Year = 1989,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUGJCVYJHZlcnNpb25YJG9iamVjdHNZJGFyY2hpdmVyVCR0b3ASAAGGoKgHCBMUFRYaIVUkbnVsbNMJCgsMDxJXTlMua2V5c1pOUy5vYmplY3RzViRjbGFzc6INDoACgAOiEBGABIAFgAdccmVsYXRpdmVQYXRoWWFsaWFzRGF0YV8QJi4uL3BhcGVyL2JpYl9jaXRhdGlvbnMvbmF0dXJlMDc2ODAucmlz0hcLGBlXTlMuZGF0YU8RAZAAAAAAAZAAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAAAAAABCRAAB/////w9uYXR1cmUwNzY4MC5yaXMAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAD/////AAAAAAAAAAAAAAAAAAEAAwAACiBjdQAAAAAAAAAAAAAAAAANYmliX2NpdGF0aW9ucwAAAgBHLzpVc2VyczplbGVuYXRoZWRoZWw6cmVzZWFyY2g6Z3gxMzE6cGFwZXI6YmliX2NpdGF0aW9uczpuYXR1cmUwNzY4MC5yaXMAAA4AIAAPAG4AYQB0AHUAcgBlADAANwA2ADgAMAAuAHIAaQBzAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIARVVzZXJzL2VsZW5hdGhlZGhlbC9yZXNlYXJjaC9neDEzMS9wYXBlci9iaWJfY2l0YXRpb25zL25hdHVyZTA3NjgwLnJpcwAAEwABLwAAFQACABP//wAAgAbSGxwdHlokY2xhc3NuYW1lWCRjbGFzc2VzXU5TTXV0YWJsZURhdGGjHR8gVk5TRGF0YVhOU09iamVjdNIbHCIjXE5TRGljdGlvbmFyeaIiIF8QD05TS2V5ZWRBcmNoaXZlctEmJ1Ryb290gAEACAARABoAIwAtADIANwBAAEYATQBVAGAAZwBqAGwAbgBxAHMAdQB3AIQAjgC3ALwAxAJYAloCXwJqAnMCgQKFAowClQKaAqcCqgK8Ar8CxAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAALG}}

@article{iaria14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...561A..99I},
	Archiveprefix = {arXiv},
	Author = {{Iaria}, R. and {Di Salvo}, T. and {Burderi}, L. and {Riggio}, A. and {D'A{\`\i}}, A. and {Robba}, N.~R.},
	Doi = {10.1051/0004-6361/201322328},
	Eid = {A99},
	Eprint = {1310.6628},
	Journal = {\aap},
	Keywords = {stars: neutron, stars: individual: GX 13+1, X-rays: binaries, X-rays: stars, ephemerides},
	Month = jan,
	Pages = {A99},
	Primaryclass = {astro-ph.HE},
	Title = {{Discovery of periodic dips in the light curve of GX 13+1: the X-ray orbital ephemeris of the source}},
	Volume = 561,
	Year = 2014,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUGJCVYJHZlcnNpb25YJG9iamVjdHNZJGFyY2hpdmVyVCR0b3ASAAGGoKgHCBMUFRYaIVUkbnVsbNMJCgsMDxJXTlMua2V5c1pOUy5vYmplY3RzViRjbGFzc6INDoACgAOiEBGABIAFgAdccmVsYXRpdmVQYXRoWWFsaWFzRGF0YV8QIi4uLy4uLy4uLy5UcmFzaC9taWxsZXIxNl9neDM0MC5iaWLSFwsYGVdOUy5kYXRhTxEBkAAAAAABkAACAAAMTWFjaW50b3NoIEhEAAAAAAAAAAAAAAAAAAAAyrj/FEgrAAA7A7gJEm1pbGxlcjE2X2d4MzQwLmJpYgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAADrw5tLUHCaNAAAAAAAAAAAAAwACAAAJIAAAAAAAAAAAAAAAAAAAAAYuVHJhc2gAEAAIAADKuTdUAAAAEQAIAADUHF7NAAAAAQAMOwO4CQAFHuoAAMAjAAIAPE1hY2ludG9zaCBIRDpVc2VyczoAZWxlbmF0aGVkaGVsOgAuVHJhc2g6AG1pbGxlcjE2X2d4MzQwLmJpYgAOACYAEgBtAGkAbABsAGUAcgAxADYAXwBnAHgAMwA0ADAALgBiAGkAYgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASACxVc2Vycy9lbGVuYXRoZWRoZWwvLlRyYXNoL21pbGxlcjE2X2d4MzQwLmJpYgATAAEvAAAVAAIAE///AACABtIbHB0eWiRjbGFzc25hbWVYJGNsYXNzZXNdTlNNdXRhYmxlRGF0YaMdHyBWTlNEYXRhWE5TT2JqZWN00hscIiNcTlNEaWN0aW9uYXJ5oiIgXxAPTlNLZXllZEFyY2hpdmVy0SYnVHJvb3SAAQAIABEAGgAjAC0AMgA3AEAARgBNAFUAYABnAGoAbABuAHEAcwB1AHcAhACOALMAuADAAlQCVgJbAmYCbwJ9AoECiAKRApYCowKmArgCuwLAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAsI=},
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201322328}}

@article{corbet10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...719..979C},
	Archiveprefix = {arXiv},
	Author = {{Corbet}, R.~H.~D. and {Pearlman}, A.~B. and {Buxton}, M. and {Levine}, A.~M.},
	Doi = {10.1088/0004-637X/719/1/979},
	Eprint = {1006.5068},
	Journal = {\apj},
	Keywords = {stars: individual: GX 13+1, stars: neutron, X-rays: stars},
	Month = aug,
	Pages = {979-984},
	Primaryclass = {astro-ph.HE},
	Title = {{Properties of the 24 Day Modulation in GX 13+1 from Near-infrared and X-ray Observations}},
	Volume = 719,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/719/1/979}}

@article{nowaksimple,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...689.1199N},
	Archiveprefix = {arXiv},
	Author = {{Nowak}, M.~A. and {Juett}, A. and {Homan}, J. and {Yao}, Y. and {Wilms}, J. and {Schulz}, N.~S. and {Canizares}, C.~R.},
	Doi = {10.1086/592227},
	Eprint = {0809.3005},
	Journal = {\apj},
	Keywords = {Accretion, Accretion Disks, Black Hole Physics, Radiation Mechanisms: Thermal, X-Rays: Binaries},
	Month = dec,
	Pages = {1199-1214},
	Title = {{Disk-dominated States of 4U 1957+11: Chandra, XMM-Newton, and RXTE Observations of Ostensibly the Most Rapidly Spinning Galactic Black Hole}},
	Volume = 689,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/592227}}

@article{hankesimple,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...690..330H},
	Archiveprefix = {arXiv},
	Author = {{Hanke}, M. and {Wilms}, J. and {Nowak}, M.~A. and {Pottschmidt}, K. and {Schulz}, N.~S. and {Lee}, J.~C.},
	Doi = {10.1088/0004-637X/690/1/330},
	Eprint = {0808.3771},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, stars: individual: HDE 226868 Cyg X-1, stars: winds, outflows, techniques: spectroscopic, X-rays: binaries},
	Month = jan,
	Pages = {330-346},
	Title = {{Chandra X-Ray Spectroscopy of the Focused Wind in the Cygnus X-1 System. I. The Nondip Spectrum in the Low/Hard State}},
	Volume = 690,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/690/1/330}}

@article{trigoboirin,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2016AN....337..368D},
	Archiveprefix = {arXiv},
	Author = {{D{\'{\i}}az Trigo}, M. and {Boirin}, L.},
	Doi = {10.1002/asna.201612315},
	Eprint = {1510.03576},
	Journal = {Astronomische Nachrichten},
	Keywords = {accretion, accretion disks, black hole physics, stars: neutron, techniques: spectroscopy, X-rays: binaries},
	Month = may,
	Pages = {368},
	Primaryclass = {astro-ph.HE},
	Title = {{Accretion disc atmospheres and winds in low-mass X-ray binaries}},
	Volume = 337,
	Year = 2016,
	Bdsk-Url-1 = {http://dx.doi.org/10.1002/asna.201612315}}

@article{verner,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...465..487V},
	Author = {{Verner}, D.~A. and {Ferland}, G.~J. and {Korista}, K.~T. and {Yakovlev}, D.~G.},
	Doi = {10.1086/177435},
	Eprint = {astro-ph/9601009},
	Journal = {\apj},
	Keywords = {ATOMIC DATA, ATOMIC PROCESSES},
	Month = jul,
	Pages = {487},
	Title = {{Atomic Data for Astrophysics. II. New Analytic FITS for Photoionization Cross Sections of Atoms and Ions}},
	Volume = 465,
	Year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/177435}}

@article{schulzsik,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160504837S},
	Archiveprefix = {arXiv},
	Author = {{Schulz}, N.~S. and {Corrales}, L. and {Canizares}, C.~R.},
	Eprint = {1605.04837},
	Journal = {ArXiv e-prints},
	Keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
	Month = may,
	Title = {{Si K Edge Structure and Variability in Galactic X-Ray Binaries}},
	Year = 2016}

@article{diaztrigowarm,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...445..179D},
	Author = {{D{\'{\i}}az Trigo}, M. and {Parmar}, A.~N. and {Boirin}, L. and {M{\'e}ndez}, M. and {Kaastra}, J.~S.},
	Doi = {10.1051/0004-6361:20053586},
	Eprint = {astro-ph/0509342},
	Journal = {\aap},
	Keywords = {X-rays: individual: EXO 0748-676, , XB 1254-690, X 1624-490, MXB 1659-298, 4U 1746-371, XB 1916-053, X-rays binaries, accretion, accretion disks},
	Month = jan,
	Pages = {179-195},
	Title = {{Spectral changes during dipping in low-mass X-ray binaries due to highly-ionized absorbers}},
	Volume = 445,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20053586}}

@article{exo0748jimenez,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...590..432J},
	Author = {{Jimenez-Garate}, M.~A. and {Schulz}, N.~S. and {Marshall}, H.~L.},
	Doi = {10.1086/374864},
	Eprint = {astro-ph/0302391},
	Journal = {\apj},
	Keywords = {Accretion, Accretion Disks, Stars: Binaries: Eclipsing, Line: Identification, Stars: Individual: Alphanumeric: EXO 0748-676, X-Rays: Binaries},
	Month = jun,
	Pages = {432-444},
	Title = {{Discrete X-Ray Signatures of a Photoionized Plasma above the Accretion Disk of the Neutron Star EXO 0748-676}},
	Volume = 590,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUGJCVYJHZlcnNpb25YJG9iamVjdHNZJGFyY2hpdmVyVCR0b3ASAAGGoKgHCBMUFRYaIVUkbnVsbNMJCgsMDxJXTlMua2V5c1pOUy5vYmplY3RzViRjbGFzc6INDoACgAOiEBGABIAFgAdccmVsYXRpdmVQYXRoWWFsaWFzRGF0YV8QIC4uL3BhcGVyL2JpYl9jaXRhdGlvbnMvdGdjYXQuYmli0hcLGBlXTlMuZGF0YU8RAXgAAAAAAXgAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAAAAAABCRAAB/////wl0Z2NhdC5iaWIAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAD/////AAAAAAAAAAAAAAAAAAEAAwAACiBjdQAAAAAAAAAAAAAAAAANYmliX2NpdGF0aW9ucwAAAgBBLzpVc2VyczplbGVuYXRoZWRoZWw6cmVzZWFyY2g6Z3gxMzE6cGFwZXI6YmliX2NpdGF0aW9uczp0Z2NhdC5iaWIAAA4AFAAJAHQAZwBjAGEAdAAuAGIAaQBiAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIAP1VzZXJzL2VsZW5hdGhlZGhlbC9yZXNlYXJjaC9neDEzMS9wYXBlci9iaWJfY2l0YXRpb25zL3RnY2F0LmJpYgAAEwABLwAAFQACABP//wAAgAbSGxwdHlokY2xhc3NuYW1lWCRjbGFzc2VzXU5TTXV0YWJsZURhdGGjHR8gVk5TRGF0YVhOU09iamVjdNIbHCIjXE5TRGljdGlvbmFyeaIiIF8QD05TS2V5ZWRBcmNoaXZlctEmJ1Ryb290gAEACAARABoAIwAtADIANwBAAEYATQBVAGAAZwBqAGwAbgBxAHMAdQB3AIQAjgCxALYAvgI6AjwCQQJMAlUCYwJnAm4CdwJ8AokCjAKeAqECpgAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKo},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/374864}}

@article{vanpeet09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...497..805V},
	Archiveprefix = {arXiv},
	Author = {{van Peet}, J.~C.~A. and {Costantini}, E. and {M{\'e}ndez}, M. and {Paerels}, F.~B.~S. and {Cottam}, J.},
	Doi = {10.1051/0004-6361/200811181},
	Eprint = {0902.4470},
	Journal = {\aap},
	Keywords = {atomic processes, stars: binaries: general, X-rays: binaries, X-rays: individuals: EXO 0748-676},
	Month = apr,
	Pages = {805-813},
	Primaryclass = {astro-ph.GA},
	Title = {{Properties of the ionised plasma in the vicinity of the neutron-star X-ray binary EXO 0748-676}},
	Volume = 497,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200811181}}

@article{king12uf,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...746L..20K},
	Archiveprefix = {arXiv},
	Author = {{King}, A.~L. and {Miller}, J.~M. and {Raymond}, J. and {Fabian}, A.~C. and {Reynolds}, C.~S. and {Kallman}, T.~R. and {Maitra}, D. and {Cackett}, E.~M. and {Rupen}, M.~P.},
	Doi = {10.1088/2041-8205/746/2/L20},
	Eid = {L20},
	Eprint = {1112.3648},
	Journal = {\apjl},
	Keywords = {accretion, accretion disks, black hole physics, X-rays: binaries},
	Month = feb,
	Pages = {L20},
	Primaryclass = {astro-ph.HE},
	Title = {{An Extreme X-Ray Disk Wind in the Black Hole Candidate IGR J17091-3624}},
	Volume = 746,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/746/2/L20}}

